A computationally efficient framework for vector representation of persistence diagrams

In Topological Data Analysis, a common way of quantifying the shape of data is to use a persistence diagram (PD). PDs are multisets of points in $\mathbb{R}^2$ computed using tools of algebraic topology. However, this multi-set structure limits the utility of PDs in applications. Therefore, in recent years efforts have been directed towards extracting informative and efficient summaries from PDs to broaden the scope of their use for machine learning tasks. We propose a computationally efficient framework to convert a PD into a vector in $\mathbb{R}^n$, called a vectorized persistence block (VPB). We show that our representation possesses many of the desired properties of vector-based summaries such as stability with respect to input noise, low computational cost and flexibility. Through simulation studies, we demonstrate the effectiveness of VPBs in terms of performance and computational cost within various learning tasks, namely clustering, classification and change point detection.

==> Experiments.tex <==
% !TEX root = arxiv_version.tex

In this section we present our experimental results to illustrate the utility of PVBs for classification, clustering and change point detection tasks. In all the experiments, our results are compared against the corresponding results produced from PIs in terms of performance and computational cost. Two of the experiments closely mimic those of Sections 6.1 and 6.4 in \cite{PI}. The experiments involve both synthetic and real datasets. On 2D datasets, we extract topological information using the Vietoris-Rips complex filtration. For large 3D datasets, we resort to the Alpha complexes to avoid computational challenges that arise from using the Vietoris-Rips complexes. To produce PIs we utilize the Matlab code publicly available at \hyperlink{https://github.com/CSU-TDA/PersistenceImages}{https://github.com/CSU-TDA/PersistenceImages}. All other implementations are performed in {\tt R}; PDs are computed using the {\tt R} package {\tt TDA}  [citation].

\subsection{Clustering using K-medoids on synthetic dataset}\label{sec1.1}
This experiment considers the synthetic dataset used in Sections 6.1 of \cite{PI} and consisting of 25 point clouds of size 500 sampled uniformly from each of the following six shapes: a unit cube, a circle of radius one half, a sphere of of radius one half, three clusters with random centers in the unit cube, three clusters each containing another set of three clusters, a torus with inner and outer diameters of one half and one respectively. Furthermore, Gaussian noise is added to each point cloud at two different levels of $\eta=0.05$ and $\eta=0.1$. Topological signatures (in the form of PVBs and PIs) are computed from PDs for homological dimensions $H0$ and $H_1$. In this experiment, the goal is to cluster the given 150 point clouds into respective 6 shape classes. 

For PIs we use are the parameter settings adopted by the authors of \cite{PI}: standard deviation $\sigma=0.1$, resolution $20\times20$ and the linear weighting function. We compute PVBs on a $6\times 6$ grid using weight function $w(x,y)=x+y$ and the values of $\alpha$ ranging in $\{0.1,0.3,0.5,0.7,0.9\}$. 

Following the approach in \cite{PI}, clustering is performed employing K-medoids method [citation]. A $150 \times 150$ matrix of pairwise distances (also called a dissimilarity matrix) between topological signatures (PVBs or PIs) and the number of clusters $K=6$ are supplied as inputs and K-medoids returns a list of cluster assignments. The performance is evaluated based on the accuracy of cluster predictions against the true cluster labels. 
%
For PVBs, several options of the length parameter $\lambda$ were used, which in general can be written in the form
\begin{eqnarray}
  \label{eq:Fij}
\lambda &=& F_{n_1, n_2}(y, \alpha) = \alpha y \left(\frac{y}{y_{max}}\right)^{n_1} \left(1-\frac{y}{y_{max}}\right)^{n_2},
\end{eqnarray}
where $\alpha\in[0;1]$ is a continuous parameter and $n_{1,2}$ are integers, and $y$ is the vector of persistence coordinates. We run K-medoids clustering algorithm and use the internal measure of Davies-Bouldin Index [citation] to select the optimal value of $\alpha$, $n_{1,2}$.

Our results are shown in figures \ref{fig:alphaPerfomance}, \ref{fig:gridPerfomance} and it is clear that the functions
\begin{eqnarray}
  \label{eq:1}
  \lambda(y) &= F_{00}(y; \alpha) = \alpha y
\end{eqnarray}
and
\begin{eqnarray}
  \label{eq:2}
  \lambda(y) = F_{01}(y; \alpha) = \alpha y\left(1-\frac{y}{y_{max}}\right)
\end{eqnarray}
give the best results.

\begin{figure}
  \centering
  \includegraphics[width=0.9\textwidth]{figures/toys_perfomance_comparison}
  \caption{Perfomance. $L_1$ metric and $5\times5$ grid are used to construct these figures}
  \label{fig:alphaPerfomance}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=0.9\textwidth]{figures/toys_perfomance_comparison_grid}
  \caption{Grid Perfomance. $L_1$ metric and $\alpha=0.75$ are used to construct these figures}
  \label{fig:gridPerfomance}
\end{figure}




Comparison of the clustering accuracy and time are given in Table \ref{six-shapes-table} and Figure \ref{six-shapes-comp-cost} below.







\begin{figure}
      \centering
    \begin{minipage}[b]{.45\textwidth}
  \centering
  \begin{tabular}{ccccc}
    \hline
    Metric & Dim & Noise & PI-Acc & PB-Acc \\ 
    \hline
    $L_1$ & $H_0$ & 0.05 & 0.933 &  \bf{0.947} \\ 
    $L_2$ & $H_0$ & 0.05 & 0.927 &   \bf{0.940} \\ 
    $L_\infty$ & $H_0$ & 0.05 & 0.940   & \bf{0.947} \\ 
    $L_1$ & $H_0$ & 0.10 & 0.953 &  \bf{0.960}\\ 
    $L_2$ & $H_0$ & 0.10 & 0.953 &  \bf{0.960} \\ 
    $L_\infty$ & $H_0$ & 0.10 & 0.960  &  0.960  \\ 
    $L_1$ & $H_1$ & 0.05 & 1.000 & 1.000 \\ 
    $L_2$ & $H_1$ & 0.05 & 1.000 & 1.000 \\ 
    $L_\infty$ & $H_1$ & 0.05 & 1.000 &  1.000 \\ 
    $L_1$ & $H_1$ & 0.10 & 0.953 & \bf{0.973} \\ 
    $L_2$ & $H_1$ & 0.10 & 0.960 & \bf{0.973}\\ 
    $L_\infty$ & $H_1$ & 0.10 & 0.960 &  0.960 \\ 
    \hline
  \end{tabular}
  \label{six-shapes-table}
        \caption{K-medoids accuracy results for PVBs and PIs}
        \label{six-shapes-table}
      \end{minipage}%
      %
      \quad
      %
    \begin{minipage}[b]{.45\textwidth}
        \centering
        \includegraphics[scale=0.5]{figures/time_complx.pdf}
        \caption{K-medoids computational costs for PVBs and PIs}
        \label{six-shapes-comp-cost}
    \end{minipage}
\end{figure}


The computational cost is the combined time (measured in seconds) to compute topological signatures and running K-medoids algorithm. The results show that K-medoids produce slightly better accuracies on PVBs. We also observe that the computational cost associated with PVBs is significantly lower despite running K-medoids for five different values of $\alpha$. 
	
\subsection{Clustering using K-medoids on real dataset}

In our second experiment, we perform clustering and shape retrieval tasks on a 3D dataset. The dataset \cite{Shrec17} consists of 100 point clouds derived from 3D scans of ten non-rigid toys and each having approximately 4000 points. All toys are scanned in ten different poses by moving various body parts around their joints (see Figures ~\ref{fig1:shrec17} and \ref{fig2:shrec17}). The dataset contains only vertex information, no triangle mesh is provided.

\begin{figure}
	\centering
		\begin{minipage}[b]{.45\textwidth}
		\centering
		\includegraphics[scale=0.5]{figures/shrec17-toys.pdf}
		\caption{Toys used for Shrec17 dataset.}
		\label{fig1:shrec17}
	\end{minipage}
%
\quad
%
	\begin{minipage}[b]{.45\textwidth}
	\includegraphics[scale=0.22]{figures/Shrec2017_sample_dataset.png}
	\caption{Sample point clouds from Shrec17 dataset. The points are colored based on $y$ and $z$ coordinates.}
	\label{fig2:shrec17}
\end{minipage}
\end{figure}

As in Section \ref{sec1.1}, we perform clustering using K-medoids algorithm. To compute PIs and PVB in this setting, we experiment with a range of values for the tuning parameters. For PIs, we select $\sigma=10^{-6}$ and a $20 \times 20$ grid. PVBs are computed on a $12\times12$ grid. All the other settings carry over from the previous section. In particular, similar to the previous experiment, we perform clustering for each homological dimension.
%
For PVB we performed a scan of the over  Davies-Bouldin Index over the parameter $\alpha$ for different parameterizations of the size function (\ref{eq:Fij}), the results are shown in Figure \ref{fig:shrec17_comparison}. As you can see, 
%
that PVBs and PIs are most discriminative for dimension $H_2$ and therefore in the following we report our results only for this dimension. Moreover, similar to the results of the previous subsection, $F_{00}$ parametrization with high value of the $\alpha$ parameter gives the best accuracy value. The Figure \ref{fig:shrec17_acc} shows a noticeable difference in accuracies between the two methods.

\begin{figure}
  \centering
  \includegraphics[width=0.9\textwidth]{figures/shreck_perfomance_comparison.png}
  \caption{Accuracy dependence of SHREC’17 dataset clustering for different topological dimensions and parametrizations of the size functions}
  \label{fig:shrec17_comparison}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[scale=0.5]{figures/cluster-shrec17-res20.pdf}
	\caption{Homological dimension used is $H_2$}
	\label{fig:shrec17_acc}
\end{figure}

The $100\times100$  dissimilarity matrix used as input for K-medoids, can also be viewed as a result of a 3D shape retrieval problem. In shape retrieval, as with clustering, no class information is allowed to be used to compute this matrix. We evaluate the retrieval performance using five standard statistics (Nearest Neighbor (NN), First-Tier (FT), Second-Tier (ST), E-Measure (E) and Discounted Cumulative Gain (DCG) [citation]) computed over the dissimilarity matrix. 

The selected dataset for our experiment was used for the 2017 Shape Retrieval Contest (SHREC) track: Point-Cloud Shape Retrieval of Non-Rigid Toys. This track invited researchers to contribute to development of new discriminative and efficient descriptors of 3D non-rigid shapes. A total of eight groups participated in this content. Each group was allowed to submit up to 6 dissimilarity matrices. We compare our results not only against the performance of PIs but also against the best results of all participants. 

\begin{figure}
	\centering
		\begin{tabular}{lccccc}
			\hline
			\hline
			\textbf{Method} & \textbf{NN}& \textbf{FT} & \textbf{ST} & \textbf{E} & \textbf{DCG}\\ 
			\hline
			\hline
			BoW-RoPS-DMF-3 & 1.0000 & 0.9778 & 0.9978 &  0.4390 &  0.9979\\ 
			BPHAPT & 0.9800 & 0.9111 & 0.9544& 0.4273&0.9743\\
			PVB & 0.9800 &	0.8378	&0.9567	&0.4351	&0.9563\\
			PI & 0.9300	&0.7589 &0.8911	&0.4180 &	0.9109\\
			MFLO-FV-IWKS &0.8900 &0.7911& 0.8589 &0.4024 &0.9038\\
			CDSPF & 0.9200 &0.6744 &0.8156 &0.4005 &0.8851\\
			SnapNet &0.8800 &0.6633 &0.8011& 0.3985 & 0.8663 \\
			AlphaVol1 &0.7900 &0.5878 &0.7578& 0.3980 &0.8145\\
			SQFD(WKS) &0.5400 &0.3111 & 0.4467 &0.2507 & 0.6032\\
			m3DSH-2 &0.4400 &0.1867& 0.2856& 0.1932 &0.4997\\
			\hline
		\end{tabular}
		\caption{Retrieval results on Shrec17. The methods are ranked according to overall performance.}
		\label{retrieval-results}
\end{figure}

We used $L_1$ distance to compute the dissimilarity matrix for PVBs and PIs. For PVBs, $\alpha=0.1$ gives a slightly better result than that of $\alpha=0.3$ for which Davies-Bouldin Index is minimum. From Figure \ref{retrieval-results}, it can be seen that our method ties for the second place with BPHAPT - we have the same NN score and outperforms in terms of ST and EE scores, while PIs deliver the fourth best result.

Furthermore, our method exhibits substantial computational advantages over both BoW-RoPS-DMF-3 and BPHAPT. For example, for BoW-RoPS-DMF-3 which utilizes the Bag-of-Words scheme, it takes 30 minutes for the codebook module to run, whereas for our method needs only about 48 seconds to compute all the topological summaries (46 seconds for PDs and 2 seconds for PVBs). In terms of data preprocessing, BPHAPT has an extra step of constructing triangular meshes using the Poisson reconstruction method, while our approach does not preprocess the data and only uses the vertex information. Finally, our method has simpler complexity with regard to the number of tuning parameters involved - we only need to choose the parameter $\alpha$ and the grid size.






%%% Local Variables:
%%% mode: latex
%%% TeX-master: "arxiv_version"
%%% End:



==> LitrReview.tex <==
% !TEX root = arxiv_version.tex

The topology diagram analysis (TDA) is one of the actively developing branches in statistics, mathematics, computer science and data science fields. The usage of the topology concepts allows one to concentrate on the most general properties of the datasets which are being analyzed and helps to understand its shape. TDA is widely used in such fields as neuroscience \cite{bendich2016persistent, 2015NatCo...6.8581N}, biology \cite{li2015identification, 2020ERL....15j4039B} , social networking \cite{carstens2013persistent}, physics \cite{donato2016persistent, 2021arXiv210312554K, 2020PhRvR...2d3308O, 2020IJMPA..3550049H}, etc.

One of the approaches used in TDA is so called persistence homology \cite{frosini1992measuring,ferri1998point, edelsbrunner2000topological, zomorodian2005computing}, where the topological information is extracted by tracking the changes of the topological features with the variation of some parameter the radius of the neighborhood, for example). The resulting information is stored in a simplex complex called the persistence diagram. This object can be later used by various computer algorithm for further processing.

In the works \cite{mileyko2011probability,Bubenik_2018, bell2019space, bubenik2019embeddings, turner2019different,Carrire2019OnTM} it was shown, however, that the space of the persistence diagrams is much more rich then usually used by the machine learning algorithm Hilbert space. For this reason same transformation of the obtained persistence diagrams to the Hilbert space is seguizes. Such transformation is usually called vectorization and a number of different approaches to this problem can be found in the literature. As an example me can list persistence landscapes~\cite{bubenik2015statistical}, persistence images~~\cite{adams2017persistence}, persistence indicator functions~\cite{rieck2019topological}, persistence curves~\cite{2019arXiv190407768C}, etc.

In our paper we will describe a novel approach, that will be called Persistence Blocks.

Some introduction can be found in this article: \cite{2017arXiv171004019C}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "arxiv_version"
%%% End:


==> Old_Theory_Section.tex <==
% !TEX root = arxiv_version.tex


%%%%%  SECTION 1  %%%%%%%%%%%

\begin{subsection}{April 9, 2020}\label{9April2020}
Let's state the notations in  \cite[last 3 lines, page 3]{CarBau} here: Two persistence diagrams $D_{g_1}$ and $D_{g_2}$  may have different numbers of points.  A partial matching $\Gamma$ between $D_{g_1}$ and $D_{g_2}$.  is a subset of  $D_{g_1}\times D_{g_2}$. It comes along with $\Gamma_1$ and 
$\Gamma_2$, where $\Gamma_1$ consists of those points in $D_{g_1}$  but not matched to a point in $D_{g_2}$  in the set $\Gamma$, and likewise for 
$\Gamma_2$.  The cost  
$c_{\infty}(\Gamma)$  is defined  on  \cite[page 4, line 8]{CarBau} as 
\begin{eqnarray}\label{0408.2}
c_{\infty}(\Gamma) \ = \ \max_{(p, q)\in \Gamma}\|p-q\|_\infty \ + \  \max_{p\in \Gamma_1} \|p -\Delta\|_{\infty} \ + \ \max_{q\in \Gamma_2} \|q-\Delta\|_{\infty},
\end{eqnarray}
where $\Delta = \{(x, x)\in \R\}$ is the diagonal. 

 The {\it bottleneck distance}  is defined on  \cite[page 4, line 9]{CarBau} as 
\begin{eqnarray}\label{0408.1} 
d_{\infty}(D_{g_1}, D_{g_2}) = \inf_\Gamma\, c_{\infty}(\Gamma). 
\end{eqnarray} 

If we let  $\Omega = \{(x, y) \in \R^2:  y > x\}$ be the region above $\Delta$ in the first quadrant of $\R^2$ and let $p = (a, b)\in \Omega$, then we can interpret the term $ \|p -\Delta\|_{\infty}$ in he above as 
\begin{eqnarray}\label{0408.6}
\|p -\Delta\|_{\infty} \  =  \  \inf\bigg\{  \| (a, b) - (x, x)\|_\infty : x \in \R\bigg\} \ = \ \frac{b-a}{2}.
\end{eqnarray}

If we let  $\Omega = \{(x, y) \in \R^2:  y > x\}$ be the region above $\Delta$ in the first quadrant of $\R^2$ and let $p = (a, b)\in \Omega$, then we can interpret the term $ \|p -\Delta\|_{\infty}$ in he above as 
\begin{eqnarray}\label{0408.6A}
\|p -\Delta\|_{\infty} \  =  \  \inf\bigg\{  \| (a, b) - (x, x)\|_\infty : x \in \R\bigg\} \ = \ \frac{b-a}{2}.
\end{eqnarray}

\ALnote{What is the difference detween these two sentences?}

{\bf Our proposed approach}  to calculate the distance between $D_{g_1}$ and $D_{g_2}$ by identifying $D_g$ as two functions (two vectors) $f_1$ and $f_2$ in the space $L^2(\Omega, w\,dA)$, where $w = w(y-x) > 0$ is a weight function on $\Omega$, and $dA = dxdy = $ the usual area measure on $\R^2$.   The identification is done in the following way:  Fix a length function $\la = \la(y-x)$ on $\Omega$.  
Let $D_g = \{(x_n, y_n): 1\leq n \leq N\}$ be a finite sequence of points in $\Omega$,  where the points $(x_n, y_n)$ are repeated according to multiplicities.  For each point $(x_n, y_n)$ in $D_g$, we let $\la_n = \la(y_n-x_n)$ and 
let $E_n$  be the subset of $\R^2$ given by
\begin{eqnarray}\label{0408.3} 
E_n  \ = \  \bigg[x_n-\frac{\la_n}{2},  \ x_n + \frac{\la_n}{2}\bigg] \times \bigg[y_n-\frac{\la_n}{2}, \ y_n + \frac{\la_n}{2}\bigg], 
\end{eqnarray} 
which  is   the square centered at $(x_n, y_n)$  with side length $\la_n$. 
Using the usual notation $\chi_{E_n} : \Omega \to \{0, 1\} $ to denote the characteristic function for $E_n$; that is,
\begin{eqnarray}\label{0408.15}
\chi_{E_n} = 1  \mbox{ on } E_n,  \mbox{ and }  \chi_{E_n} = 0  \mbox{ on } \Omega \setminus E_n.
\end{eqnarray}
In terms of the characteristic functions  $\chi_{E_n} $ for each point $(x_n, y_n)$ in the persistence diagram $D_g$, 
\begin{eqnarray}\label{0408.4}
\mbox{ we identify \ } D_g  \ \mbox{ as  the  function } f = \sum_{n= 1}^N \, \chi_{E_n} \ \mbox{in} \ L^2(\Omega, wdA).
\end{eqnarray}
We define the metric between two persistence diagrams  $D_{g_1}$ and $D_{g_2}$, which are identified as two functions $f_1$ and $f_2$ respectively, by 
\begin{eqnarray}\label{0408.5}
d(D_{g_1}, D_{g_2}) \  =  \ \|f_1 - f_2\| \ = \ \bigg( \int_\Omega |f_1 - f_2|^2 \, wdA \bigg)^{\frac{1}{2}}. 
\end{eqnarray} 


However, this norm $\|\cdot \|$  that we defined in (\ref{0408.5}) does not give a metric $d$ that is equivalent to the bottleneck distance given by (\ref{0408.1}).  This should not be surprising. Intuitively, the bottleneck distance is defined in terms of the  supremum norm $\|\cdot \|_\infty$, which is not equivalent to any Hilbert norm  (the norm that is induced by an inner product). Here two metrics $d_1, d_2$ on the same set $X$ are said to be {\it equivalent} if there is a positive 
  $\alpha$  such that 
\begin{eqnarray}\label{0408.7} 
\frac{1}{\alpha}\, d_1 (f, g) \leq d_2 (f, g)  \leq \alpha \, d_1(f, g) \ \ \mbox{  for all } f, g \in X. 
\end{eqnarray}


Returning to our discussion of persistence diagrams, the inequality in (\ref{0408.7}) is translated into 
\begin{eqnarray}\label{0408.16}
\frac{1}{\alpha}\, d_\infty (D_{g_1}, D_{g_2}) \leq  \|f_1 - f_2\|   \leq \alpha \, d_\infty (D_{g_1}, D_{g_2}) \ \ \mbox{  for all }  D_{g_1}, D_{g_2}
\end{eqnarray}

   Note that  a norm is equivalent to a  Hilbert norm iff every closed subspace is complemented.  However $\|\cdot \|_\infty$ does not have this property.
Even though the bottleneck distance is not precisely given by $\|\cdot \|_\infty$, it is defined on finite sequences of points in $\Omega$ in terms of $\|\cdot \|_\infty$. Thus it inherits too much property of $\|\cdot \|_\infty$ for the bottleneck distance to be equivalent to a Hilbert norm. Thus, {\it the bottleneck distance is never equivalent to a Hilbert norm of any kind. In other words,  it is hopeless to have (\ref{0408.16}) hold true for any Hilbert norm $\|\cdot\|$. } 


\begin{example} \label{0408.A} {\rm Take $\la \equiv 1$, and  $w  \equiv 1$,  and $D_{g_1} = \{(1,6)\} \cup \{(n^2,  n^2+2): 1 \leq n \leq N\}$  where $N \geq 2$ is a fixed integer,  and  $D_{g_2} = \{(1,6)\}.$ Thus we take 
\begin{eqnarray}\label{0408.8}
\Gamma = \bigg\{ \left( (1,6), (1, 6)\right)  \bigg\}
\end{eqnarray}
 to calculate the bottleneck distance, and so we have 
 \begin{eqnarray}\label{0408.10}
 \Gamma_1 = \{(n^2,  n^2+2): 1 \leq n \leq N\} \ \mbox{and} \ \Gamma_2 =\emptyset.
\end{eqnarray} 
Hence, by (\ref{0408.1}) and (\ref{0408.6}) (CHECK reference - 0408.6 or 0408.6A) we have 
\begin{eqnarray}\label{0408.9}
d_{\infty} ( D_{g_1}, D_{g_2} ) =  \inf_\Gamma\, c_\infty(\Gamma) \ = \  \max_{p\in\Gamma} \|p-\Delta\|_\infty = \frac{(n^2+2)-n^2}{2} = 1.
\end{eqnarray}
However  (\ref{0408.5}) gives 
\begin{eqnarray}\label{0408.11}
d(D_{g_1}, D_{g_2})^2  &  =  &  \  \int_\Omega |f_1 - f_2|^2 \, wdA   \\  \notag
                                 &  =  & \ \sum_{n=1}^N \, |\chi_{E_n}|^2 wdA.  \\ \notag
                                 &  = & \ \sum_{n=1}^N \mbox{Area}(E_n)   =  \ \sum_{n=1}^N 1 =   \ N,
\end{eqnarray} 
which goes to $\infty$ as $N$ goes to $\infty$.  }
\end{example}


\begin{example} \label{0408.B} {\rm Take $\la \equiv 1$, and  $w  \equiv 1$,  and $D_{g_1} = \{(N, N+1)\}$  where $N \geq 2$ is a fixed integer,  and  $D_{g_2} = \{(1,2)\}.$ Thus we have only one choice of $\Gamma$, which is
\begin{eqnarray}\label{0408.12}
\Gamma = \bigg\{ \bigg( (1,2), \ (N, N+1)\bigg)  \bigg\}, 
\end{eqnarray}
and so 
 \begin{eqnarray}\label{0408.13}
 \Gamma_1 = \Gamma_2 =\emptyset.
\end{eqnarray} 
Hence, by (\ref{0408.1}) and (\ref{0408.6}) we have 
\begin{eqnarray}\label{0408.14}
d_{\infty} ( D_{g_1}, D_{g_2} ) = \| (N, N+1) - (1, 2)\|_\infty = N-1, 
\end{eqnarray}
which goes to $\infty$   as $N$ goes to $\infty$. 
However  (\ref{0408.5}) gives 
\begin{eqnarray}\label{0408.18}
d(D_{g_1}, D_{g_2})^2  &  =  &  \  \int_\Omega |f_1 - f_2|^2 \, wdA  \  = \ \la^2 + \la^2  = 2. 
\end{eqnarray} 
}
\end{example} 



From Examples \ref{0408.A} and \ref{0408.B}, we see that  no positive  constant $\alpha$ can make (\ref{0408.16}) hold true. In other words, 
$d$ and $d_\infty$ are not equivalent metrics on the persistence diagrams.

{\bf Conclusions.}  
\begin{enumerate}
\item[1.]  From Examples  \ref{0408.A} and \ref{0408.B}, we  cannot hope to define a Hilbert norm that gives an metric that is equivalent to the bottleneck distance $d_{\infty}.$
\item[2.]  From Examples  \ref{0408.A} and \ref{0408.B}, it seems that the metric $d$ given by (\ref{0408.5}) has its advantage  over the bottleneck distance 
$d_\infty$  as given by (\ref{0408.1}).  After all, $d$ comes from a desirable Hilbert norm.  Should we give more convincing proof that $d$ is a good choice over 
$d_{\infty}$, perhaps at least in some cases? 
\item[3.] It seems that it is more efficient to calculate $d$ given by (\ref{0408.5}) than $d_\infty$  given by (\ref{0408.1}). Reason: 
Suppose $d_{g_1}$ is a set of $n$ ordered pairs in $\Omega$ and $d_{g_2}$ is a set of $m$ ordered pairs in $\Omega$, where $m \geq n$.  Thus there are at least 
$P(m, n) = \frac{m!}{(m-n)!}$   possible partial matchings $\Gamma$, which is a huge number when $m$ and $n$ are both large.  So the term the infimum 
$\inf_\Gamma$  in the definition of $d_\infty$  in  (\ref{0408.1}) is hard to compute. Should we devise an algorithm for computing $d$ given by (\ref{0408.5}) to make computation easy? For example, in Examples \ref{0408.A} and \ref{0408.B} we evaluate the integrals in (\ref{0408.5}) by computing simple arithmetics. 
So, can integral in (\ref{0408.5})  be rephrased in terms of simple arithmetics for  the computer to evaluate? 
\end{enumerate}

\end{subsection}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%      SECTION 2      %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{subsection}{May 17, 2020}\label{17May2020}
In this section, we continue  our discussion in the same setting as in Section \ref{9April2020}. But we change the definition of $\Omega$ to $\Omega = \{(x, y) :  x > 0 \mbox{ and } y > 0\}$ be the positive first quadrant of the $x, y$-plane,   Let   $P(\Omega)$  be  the collection of all persistence diagrams $D = \{(x_n, y_n) \in \Omega:  1 \leq n \leq N\}$ where $N \geq 1$ is an integer.  Let  $\la : \Omega \to (0,\infty)$ be a continuous length function defined for each  point $(x, y)$  in $\Omega$. Using this length function $\la$, we define for each point $(x, y)$ in $\Omega$ a square  $E$ lying inside 
$\Omega$,  centered at $(x, y)$ with side length  $\la  = \la(x, y),$ given  by 
\begin{eqnarray}\label{0514.1}
E = E(x, y) =\left[x-\frac{\la}{2},\,  x+ \frac{\la}{2}\right] \times \left[y-\frac{\la}{2},\,  y+\frac{\la}{2}\right].  
\end{eqnarray}



Let $w: \Omega \to  (0,\infty)$ be a continuous weight function on $\Omega,$  and consider the weighted area measure $wdA$ on $\Omega$ and its corresponding Hilbert space $L^2(wdA)$. 
 Define the map  $\rho:  P(\Omega) \to L^2(wdA)$ that identifies each persistence diagram $D$ as a function, or a vector, in $L^2(wdA)$ by taking 
\begin{eqnarray}\label{0513.1}
\rho(D) = \rho\{(x_n, y_n) \in \Omega:  1 \leq n \leq N\} = \sum_{n=1}^N \chi_{E_n}, 
\end{eqnarray}
where 
$E_n = E(x_n, y_n)$ 
is the square in $\Omega$ centered at $(x_n, y_n)$ with side length $\la_n = \lambda (x_n, y_n)$, as  given by (\ref{0514.1}) above.

Before we proceed further, we first investigate how two squares overlap in the following lemma, which is obvious if we draw the pictures of the two squares. 


%%%%%%%%  Lemma 2.1  %%%%%%%%%

\begin{lemma}\label{0511.A}
Let  $E$ and $E'$ be two squares  with same side lengths $\la$ and $\la'$, centered at $(x, y)$ and $(x', y')$ respectively. We have the following Statements. 
\begin{enumerate}
\item[(1)] {\rm Area}$(E\cap E') > 0 $ if and only if $\displaystyle{ \|(x, y) - (x', y')) \|_\infty \  <  \ \frac{\la+\la'}{2};}$   
\item[(2)] If {\rm Area}$(E\cap E') > 0 $, then $${\rm Area}(E\cap E')  = \bigg( \frac{\la+\la'}{2}-|x-x'|\bigg)\bigg( \frac{\la+\la'}{2}-|y-y'|\bigg);$$
  \ \item[(3)]  If {\rm Area}$(E\cap E') > 0 $, then  
  \begin{eqnarray}\notag
  &   & {\rm Area}(E\setminus E') \\ \notag
&  = &  \la^2  -  {\rm Area} (E\cap E') \\ \notag
 & = &  \la^2-  \bigg( \frac{\la+\la'}{2}-|x-x'|\bigg)\bigg( \frac{\la+\la'}{2}-|y-y'|\bigg) \\ \notag
 & = & \la^2 - \bigg( \frac{\la+\la'}{2}\bigg)^2 + \bigg( \frac{\la+\la'}{2}\bigg)|x- x'| + \bigg( \frac{\la+\la'}{2}\bigg)|y-y'|    - |x-x'|\, |y-y'|. 
 \end{eqnarray}
 \item[(4)] {\rm Area}$(E\cup E') = \la^2+ {\la'}^2$ when  $\displaystyle{ \|(x, y) - (x', y')) \|_\infty \ \geq \  \frac{\la+\la'}{2}.}$
\end{enumerate} 
\end{lemma} 



Any function  $f: \Omega \to \R$ induces a  map $\tilde{f}$ on $\rho(P(\Omega))$ by 
\begin{eqnarray}\label{0512.1}
\tilde{f}(\rho (D)) =   \tilde{f} \bigg( \sum_{n=1}^N \chi_{E_n} \bigg) = \sum_{n=1}^N f(x_n, y_n) \chi_{E_n}, 
\end{eqnarray}
which is called a {\it persistence surface} in \cite[Definition 1, page 5]{AEKNP}.

 We now show that this function $\tilde{f}$ preserves continuity of the persistence diagrams. 
To do that, we first need  a topology on $P(\Omega)$.  For two persistence diagrams $D = \{(x_n, y_n) \in \Omega:  1 \leq n \leq N\} $ 
and $D' = \{(x_n', y_n') \in \Omega:  1 \leq n \leq N\} $ in $P(\Omega)$, both of which have the same number $N$ of points in $\Omega$, we 
define their  $p$-Wasserstein distance $W_p(D, D')$ , where $1\leq p < \infty$, by 
\begin{eqnarray}\label{0514.2}
&  & W_p(D, D') \\  \notag
&= &  \inf\bigg\{ \bigg( \sum_{n=1}^N \|(x_n\,  y_n) -  (x_{\sigma(n)}', y_{\sigma(n) }')\|_\infty^p \bigg)^{1/p} \, \bigg|\,  \sigma \text{ is a bijection on } \{1, 2, \ldots N\} \bigg\}.
\end{eqnarray}



%%%%%%%%%    Proposition 2.2  %%%%%%%%%%
 
\begin{proposition}\label{0512.A}
For any continuous map $f: \Omega \to \R$, the  composite map $\tilde{f}\circ \rho :  P(\Omega) \to L^2(wdA)$ given by (\ref{0512.1})  is continuous with respect to $W_p(D, D')$ for any $p$ with $1\leq p < \infty.$ (and indeed for all $p >0$.) 
\end{proposition}

\begin{proof}
Fixing a persistence diagram $D = \{(x_n, y_n) \in \Omega:  1 \leq n \leq N\} $  in $ P(\Omega) $ we need to show that $\tilde{f}\circ \rho$ is continuous at $D$. Since $D$  contains finite number of points, there is a compact subset $K$ in $\Omega$ containing all squares $E_n$ where $1 \leq n \leq N$. 

Let $c = \min\{\la_n = \la(x_n, y_n) : (x_n, y_n)\in D\} > 0$. 
Let $M  > 0$ so that 
\begin{eqnarray}\label{0515.1}
 &   &  M \geq  \max\{|f(x,y)|:  (x, y) \in K\}, \ \mbox{and} \\ \label{0515.3}
 &  & M \geq  \max\{w(x,y):  (x, y) \in K\},  \ \mbox{and} \\ \label{0515.4}
 &   &  M \geq  \max\{\la(x,y):  (x, y) \in K\}.
\end{eqnarray}
  Suppose $D'=\{(x_n', y_n') \in \Omega:  1 \leq n \leq N\}$ is a persistence diagram with the same number points as in $D$ satisfying  $|x_n-x_n'| < c$ and $|y_n - y_n'| < c$.  We first need an estimation on  the norm $\|\cdot \|$ in $L^2(wdA)$.


\begin{eqnarray}\label{0512.2}
&  &  \|\tilde{f}(\rho(D) ) - \tilde{f}(\rho(D')) \| \\ \notag
& = &\bigg\| \sum_{n=1}^N f(x_n, y_n)\chi_{E_n} -  \sum_{n=1}^N f(x_n', y_n')\chi_{E_n'}\bigg\|  \\ \notag
& \leq & \sum_{n=1}^N \| f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}\| \\ \notag
& = & \sum_{n=1}^N  \left( \int_\Omega | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, wdA\right)^{1/2}
\end{eqnarray}
We now focus on the above integral. 
\begin{eqnarray}\label{0512.3}
& & \ \ \int_\Omega | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2\,  wdA \\ \notag
&= & \ \ \int_{E_n \cup E_n'}\,  | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, wdA \\ \notag
&\leq & \  \ Mf(x_n, y_n)^2\, \mbox{Area}(E_n \setminus E_n') +  M (f(x_n, y_n) - f(x_n', y_n'))^2 \, \mbox{Area} (E_n \cap E_n') + \\ \notag
&   & + M f(x_n', y_n')^2 \mbox{Area} (E_n' \setminus E_n), \ \mbox{ by  (\ref{0515.3}).} \\ \notag
&\leq & \  M^3 \mbox{Area}(E_n \setminus E_n')  +  M (f(x_n, y_n) - f(x_n', y_n'))^2 \, \mbox{Area} (E_n \cap E_n') \\ \notag 
&  & +  M^3\mbox{Area}(E_n' \setminus E_n),  \ \mbox{ by  (\ref{0515.1}).}\\ \notag
\end{eqnarray}
We now use  Statement (3) of Lemma \ref{0511.A} and (\ref{0515.4}) to estimate Area$(E_n \setminus E_n')$ to get 
\begin{eqnarray}\label{0515.5}
{\rm Area}(E_n \setminus E_n')  \ \leq \   \la_n^2 - \bigg( \frac{\la_n+\la_n'}{2}\bigg)^2 + M|x- x'| +M|y-y'|,   \\ \notag
\end{eqnarray}
and by interchanging $E_n$ and $E_n'$,  we have 
\begin{eqnarray}\label{0515.6}
{\rm Area}(E_n' \setminus E_n) \  \leq  \   {\la_n'}^2 - \bigg( \frac{\la_n+\la_n'}{2}\bigg)^2 + M|x- x'| +M|y-y'|,   \\ \notag
\end{eqnarray}
Similarly using Statement (2) of Lemma \ref{0511.A} and (\ref{0515.4}) to estimate Area$(E_n \cap E_n')$, we get 
\begin{eqnarray}\label{0515.7}
{\rm Area}(E_n\cap E_n') \leq   (M-|x-x'|)(M-|y-y'|) \leq M^2.  \\ \notag
\end{eqnarray}


We now use the estimations in (\ref{0515.5}), (\ref{0515.6}), and (\ref{0515.7}) to continue our estimation in (\ref{0512.3}). 
\begin{eqnarray}\label{0515.2} 
& & \ \ \int_\Omega | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, wdA \\ \notag
& \leq & M^3\left( \la_n^2 +{\la_n'}^2  - \left( \frac{\la_n + \la_n'}{2} \right)^2 \right)       \ + \ 2M^4\left(|x_n-x_n'| + |y_n-y_n'|\right) \ +  \                              \\  \notag
& &  + M^3\left(f(x_n, y_n)  - f(x_n' - y_n')\right)^2.  \\ \notag
& = & M^3 \left( \frac{\la_n - \la_n'}{2} \right)^2       \ + \ 2M^4\left(|x_n-x_n'| + |y_n-y_n'|\right) \ +  \ M^3\left(f(x_n, y_n)  - f(x_n' - y_n')\right)^2. 
\end{eqnarray}

To finish the proof for continuity,  let $\epsilon >0$.  Since $\la $ is uniformly continuous on the compact set $K$ which contains all squares $E_n$ and $E_n'$, there exists $\delta_1>0$  such that for any two points  $(x, y)$ and $(a,b)$  in $K$ with $\| (x, y) - (a, b)\|_\infty < \delta_1$, then 
\begin{eqnarray}\label{0515.8}
|\la(x, y) - \la(a, b)|   \ < \ \frac{\epsilon}{M^{3/2}N}  
\end{eqnarray}

Similarly, $f$ is also uniformly continuous on the compact set $K$, and so there exists $\delta_2 >0$ such that for any two points  $(x, y)$ and $(a,b)$  in $K$ with $\| (x, y) - (a, b)\|_\infty < \delta_2$, then 
\begin{eqnarray}\label{0515.14}
|f(x, y) - f(a, b)|   \ < \ \frac{\epsilon}{2M^{3/2}N}  
\end{eqnarray}


Having chosen $\delta_1$, we now choose  a $\delta$ with
\begin{eqnarray}\label{0515.9}
0 < \delta < \min\left\{c, \, \delta_1,\,  \delta_2,\,   \frac{\epsilon^2}{12N^2M^4}\right\}.  
\end{eqnarray}  
Hence  if  $W_p(D, D') < \delta$ then there is a bijection $\sigma :\{1, 2, \ldots, N\} \to \{1, 2, \ldots, N\}$ such that 
\begin{eqnarray}\label{0515.10} 
\bigg( \sum_{n=1}^N \|(x_n\,  y_n) -  (x_{\sigma(n)}', y_{\sigma(n)' })\|_\infty^p \bigg)^{1/p} \ < \delta.
\end{eqnarray}
Hence there is a bijection $\sigma$ such that 
\begin{eqnarray}\label{0515.11}
\|(x_n\,  y_n) -  (x_{\sigma(n)}', y_{\sigma(n) }')\|_\infty \ < \ \delta.
\end{eqnarray}
Hence, without loss of generality, by relabelling $(x_n', y_n')$ if necessary, we can assume 
\begin{eqnarray}\label{0515.12}
\|(x_n\,  y_n) -  (x_{n}', y_n')\|_\infty \ < \ \delta. 
\end{eqnarray}
With this assumption,  we  now use (\ref{0515.8}), (\ref{0515.14}), and (\ref{0515.12}) to continue our estimation in (\ref{0512.2}). 
\begin{eqnarray}\label{0515.15}
& & \ \ \int_\Omega | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \,wdA \\ \notag
& \leq &  M^3\left(\frac{\epsilon}{2M^{3/2}N}\right)^2 \  + \ 4M^4\delta \ + \ M^3\left( \frac{\epsilon}{2M^{3/2}N}\right)^2\\ \notag
& < & \frac{\epsilon^2}{4N^2}  \ + \ 4M^4 \frac{\epsilon^2}{12N^2M^4} \ + \  \frac{\epsilon^2}{4N^2}, \text{ \ by (\ref{0515.9})}  \\ \notag
& < &  \frac{\epsilon^2}{N^2}.
\end{eqnarray}
Hence  by putting the estimate in (\ref{0515.15}) into  (\ref{0512.2}), we have  
 \begin{eqnarray}\label{0515.16}
 \|\tilde{f}(\rho(D) ) - \tilde{f}(\rho(D')) \| \ < \ \sum_{n=1}^N  \sqrt{\frac{\epsilon^2}{N^2}} \ = \ \epsilon,
\end{eqnarray} 
which concludes our proof.
\end{proof}



We now prove the converse of Proposition \ref{0512.A}.

%%%%  Proposition 2.3   %%%%%%%%

\begin{proposition}\label{0516.A}
For any map $f: \Omega \to \R$, if the  composite map $\tilde{f}\circ \rho :  P(\Omega) \to L^2(wdA)$ given by (\ref{0512.1})  is continuous with respect to $W_p(D, D')$ for some $p$ with $1\leq p < \infty,$ then $f$ is continuous.
\end{proposition} 

\begin{proof} Let $\epsilon >0$ and $(x, y) \in \Omega$. We are to show there is a  $\delta > 0$ so that $|f(x', y')- f(x, y)| < \epsilon$ whenever $\|(x, y)- (x', y')\|_\infty< \delta$.  

Let $K$ be a compact subset of $\Omega$ whose interior int\,$K$ contains the compact square $E(x, y)$.  By the continuity of  the side length function $\la : \Omega \to (0, \infty).$ there exists a $\delta_1 > 0$ such that if $\|(x', y') - (x, y)\|_\infty < \delta_1$, then the square 
\begin{eqnarray}\label{0516.1}
E(x', y') \subset K,  \mbox{\ and} \ {\rm Area}\left(E(x,y) \cap E(x',y') \right) > \frac{1}{2}{\rm Area}\left(E(x,y)\right).
\end{eqnarray}

Since $K$ is compact, and $\la$ and $w$ are continuous on $K$, there exists a $\mu >0$ such that 
\begin{eqnarray}\label{0516.2}
\mu \,  < \, \min\{\la(a, b): (a,b) \in K\} \ \mbox{ \ and \ } \mu \, < \, \min\{ w(a, b):  (a, b) \in K\}.
\end{eqnarray}


Since $\tilde{f}\circ \rho$ is continuous, there is a $\delta_2> 0$ such that if $D = \{(x, y)\}$ and $D' = \{(x', y')\}$ are two persistence diagrams with $W_p(D, D') < \delta_2$ then   $\| \tilde{f}\circ \rho(D) - \tilde{f}\circ \rho(D')\| \, < \, \frac{\epsilon\mu^{3/2}}{\sqrt 2}.$  

Let $\delta = \min\{\delta_1, \delta_2\}$. If $\|(x', y') - (x, y)\|_\infty  < \delta$, then it is clear that $W_p(D, D') = \|(x', y') - (x, y)\|_\infty < \delta_2$, and hence
\begin{eqnarray}\label{0516.3}
\| \tilde{f}\circ \rho(D) - \tilde{f}\circ \rho(D')\|^2    \ < \ \frac{\epsilon^2\mu^{3}}{2}. 
\end{eqnarray}
It follows that from the definition of $\tilde{f}\circ \rho$ in (\ref{0512.1}) that 
\begin{eqnarray}\label{05.16.4}
 \ \  \ \int_{E(x, y)\cap E(x', y')} \, |f(x, y)- f(x', y')|^2\, wdA \ \leq \ \| \tilde{f}\circ \rho(D) - \tilde{f}\circ \rho(D')\|^2 \ < \  \frac{\epsilon^2\mu^{3}}{2}. 
\end{eqnarray}
We now obtain a lower bound for the above integral using (\ref{0516.2}) 
\begin{eqnarray}\label{05.16.5}
&  & \int_{E(x, y)\cap E(x', y')} \, |f(x, y)- f(x', y')|^2\, wdA \\ \notag
 & \geq  & \ \mu \left(f(x, y)- f(x', y')\right)^2 {\rm Area}\left(E(x,y)\cap E(x', y')\right) \\ \notag
 & \leq  & \mu \left( f(x, y)- f(x', y')\right)^2\frac{\mu^2}{2},   \mbox{ by  (\ref{0516.1})  and (\ref{0516.2})   } 
\end{eqnarray}
Combining the two chain of inequalities in (\ref{05.16.4}) and (\ref{05.16.5}), we get 
\begin{eqnarray}\label{05.16.6}
|f(x, y) - f(x', y')| < \epsilon,
\end{eqnarray}
as desired.
\end{proof} 

We now turn our attention to the continuity of the identification map $\rho:  P(\Omega) \to L^2(wdA)$ relative to the $1/2$-Wasserstein distances between persistence diagrams in $P(\Omega).$

Following \cite[Theorems 4, 9, 10]{AEKNP},  we prove an analogous result here:


%%%%%%   Proposition 2.4  %%%%%%%%%

\begin{proposition}\label{0510.A}
Suppose the side-length function $\lambda: \Omega \to (0, \infty)$ is bounded and Lipchitz with respect to the sup-norm on $\Omega$, and  the weight function $w: \Omega \to (0, \infty)$ is bounded. Let  $M>0$ such that 
for all $(x,y), (x',y')$ in $\Omega$, 
\begin{eqnarray} \label{0517.1}
&  & |\la(x, y) - \la(x', y')| \leq M\|(x,y)-(x',y')\|_\infty, \ \mbox{and} \\ \label{0517.9}
& &   |\la(x, y) | \leq M, \mbox{and} \  |w(x, y) | \leq M. 
\end{eqnarray}
The identification $\rho$ is stable with respect to the $1/2$-Wasserstein distances between persistence diagrams. Indeed we have 
\begin{eqnarray}\label{0510.3}
\ \ \ \ \  \|\rho(D)-\rho(D')\|  
& \leq & \sqrt{ \max\left\{ 2M^2 (M+2),  4M\right\}}\,W_{1/2}(D, D')^{1/2}. 
\end{eqnarray}
\end{proposition}


\begin{proof} 
Let $D= \{(x_n, y_n): 1 \leq n \leq N\}$ and $D' = \{(x_n', y_n'): 1\leq n \leq N\}$, and $E_n = E(x_n, y_n), $ and $E_n' = (x_n', y_n')$ be the squares given by 
(\ref{0514.1}).  
For any bijection $\sigma : \{1, 2, \ldots N\} \to \{1, 2, \ldots N\}$, we have 
\begin{eqnarray}\label{0510.4}
\| \rho(D) - \rho(D') \| \ = \  \bigg\|\sum_{n=1}^N \chi_{E_n} - \sum_{n=1}^N \chi_{E_{\sigma(n)}'}\bigg\|
\ \leq \ \sum_{n=1}^N \|\chi_{E_n} - \chi_{E_{\sigma(n)}'}\| \\ \notag
\end{eqnarray}


By renaming our integers $n$ in $x_n'$ if necessary, we can assume,  without loss of generality,  $\sigma(n) = n$ for the sake of notational simplicity.  Then we write set  $\{1, 2, \ldots, N\}$ into the disjoint union of two subsets $A,  B$ where $A$ consists of those integers $n$ such that 
\begin{eqnarray}\label{0517.3}
 \ \ \ \ \ A \ = \left\{n \ : \ 1\leq n \leq N \ \mbox{and} \ \|(x_n, y_n) - (x_{n}', y_{n}')\|_\infty \ <   \ \frac{\la(x, y) + \la(x', y')}{2}\right\}, 
\end{eqnarray}
and 
\begin{eqnarray}\label{0517.4}
B = \{1, 2, \ldots, N\} \setminus A.
\end{eqnarray}


To estimate the norm under the summation sign in  (\ref{0510.4}), we consider the two cases, depending on whether $n \in A$ or $n\in B$. First we use Lemma \ref{0511.A} to see that if $n\in A$ then

\begin{eqnarray}\label{0517.15}
&   &  \|\chi_{E_n} - \chi_{E_{n}'}\|^2   \\ \notag
& =  &  \int_\Omega  |\chi_{E_n} - \chi_{E_{n}'}|^2\, wdA \\ \notag
 & =  &  \int_{E_n \setminus  E_{n}'} \, wdA \ + \  \int_{E_n' \setminus  E_{n}}\, wdA \\ \notag
& \leq  &  M \mbox{Area}(E_n\setminus E_n') + M  \mbox{Area}(E_n' \setminus E_n)  
\end{eqnarray}
To continue our estimation, we write $\la_n = \la(x_n, y_n)$ and $\la_n' = \la(x_n', y_n')$. It follows from Statement (3) of Lemma \ref{0511.A} that  for any $n\in A$, 
\begin{eqnarray}\label{0517.19}
&   &  \|\chi_{E_n} - \chi_{E_{n}'}\|^2   \\ \notag
 & \leq & M\left(  \la_n^2 - \bigg( \frac{\la_n+\la_n'}{2}\bigg)^2 + \bigg( \frac{\la_n+\la_n'}{2}\bigg)|x_n- x_n'| + \bigg( \frac{\la_n+\la_n'}{2}\bigg)|y_n-y_n'| \ \right)+ \  \\  \notag
 &     & M\left(  \la_n'^2 - \bigg( \frac{\la_n+\la_n'}{2}\bigg)^2 + \bigg( \frac{\la_n+\la_n'}{2}\bigg)|x_n- x_n'| + \bigg( \frac{\la_n+\la_n'}{2}\bigg)|y_n-y_n'| \right) \\ \notag
  & \leq  & M\left( \frac{|3\la_n +\la_n'|\,|\,|\la_n-\la_n'| }{4}  + M|x_n- x_n'| + M|y_n-y_n'| \ \right) \ + \  \\  \notag
 &     & M\left(  \frac{|3\la_n' +\la_n|\,|\la_n'-\la_n| }{4}   + M|x_n- x_n'| + M|y_n-y_n'| \right),  \mbox{ by (\ref{0517.9})}   \\ \notag
& \leq & 2M^2\left( |\la_n'-\la_n|   + |x_n- x_n'| + |y_n-y_n'| \right),  \mbox{ by (\ref{0517.9})}   \\  \notag
&\leq  & 2M^2\left( M\|(x_n, x_n') - (y_ n, y_n')\|_\infty + |x_n- x_n'| + |y_n-y_n'| \right),  \mbox{ by (\ref{0517.1})}  \\ \notag
&\leq & 2M^2 (M+2) \|(x_n, x_n') - (y_ n, y_n')\|_\infty.
\end{eqnarray}

We now turn our attention to the case when $n$ is not in $A$.  It follows from Statement (4) of Lemma \ref{0511.A} that for any integer $n \in B$, 
\begin{eqnarray}\label{0517.16}
&  &  \|\chi_{E_n} - \chi_{E_{n}'}\|^2 \ =  \  \mbox{Area}(E_n) + \mbox{Area}(E_n')  = \la_n^2 + \la_n'^2. \\ \notag
&\leq &  (\la_n+\la_n')^2  \ \leq \ 2M(\la_n +\la_n')  \mbox{ by (\ref{0517.9})}\\ \notag
&\leq & 4M\|(x_n, x_n') - (y_ n, y_n')\|_\infty   \mbox{ by Statement (1) of Lemma \ref{0511.A} for } b\in B.
 \end{eqnarray}

Using (\ref{0517.19}) and (\ref{0517.16}), we continue our estimation in (\ref{0510.4}):   
\begin{eqnarray}\label{0517.18}
&     &  \| \rho(D) - \rho(D') \|  \\ \notag
&  \leq & \sum_{n\in A} \|\chi_{E_i} - \chi_{E_{\sigma(n)}'}\|  \ + \  \sum_{n\in B} \|\chi_{E_i} - \chi_{E_{\sigma(n)}'}\|  \\ \notag
& \leq & \sum_{n\in A } \sqrt{ 2M^2 (M+2) \|(x_n, x_n') - (y_ n, y_n')\|_\infty}
 \ + \ \sum_{n\in B }   \sqrt{4M\|(x_n, x_n') - (y_ n, y_n')\|_\infty }       \\ \notag
 &\leq & \sqrt{ \max\left\{ 2M^2 (M+2),  4M\right\}} \sum_{n=1}^N \, \sqrt{\|(x_n, x_n') - (y_ n, y_n')\|_\infty }  \\ \notag
  &= & \sqrt{ \max\left\{ 2M^2 (M+2),  4M\right\}} \sum_{n=1}^N \, \sqrt{\|(x_n, x_n') - (y_ n, y_n')\|_\infty } 
\end{eqnarray}
Since (\ref{0517.18}) holds true for all bijections $\sigma$  giving (\ref{0510.4})
we can take infimum  over all bijections $\sigma$ in (\ref{0517.18}) and conclude that 
\begin{eqnarray}\label{0517.20}
 \| \rho(D) - \rho(D') \|  \ \leq \  \sqrt{ \max\left\{ 2M^2 (M+2),  4M\right\}} \,W_{1/2}(D, D')^{1/2},
\end{eqnarray}
which finishes our proof.
\end{proof}

\bigskip


{\bf Problem 2A.}  We have to give two examples to show that the hypotheses  on $\la$ and $w$ in Proposition \ref{0510.A} are  necessary for the proposition to hold.  Do we have uniformly continuous $f$ but not uniformly continuous $\tilde{f}\circ \rho$ in each of the following cases.
\begin{enumerate}
\item[(1)]  $f(x, y) = \la(x,y) = y/2$ and $w \equiv 1.$
\item[(2)]  $f(x, y) = w(x,y) \equiv 1$ and $\la (x, y) = y^2/2$.
\item[(3)]  $f(x, y) = x+y$, \ $ w(x, y)  \equiv 1$, and $\la (x, y) = y/2$.
\end{enumerate}

\bigskip

\end{subsection}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%     SECTION 3    %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{subsection}{May 26, 2020}\label{26May2020}

In this section we follow our line of research in Section \ref{17May2020}. To be more specific, we prove give a sufficient condition for  the  composite map $\tilde{f}\circ \rho :  P(\Omega) \to L^2(wdA)$ in Proposition \ref{0512.A} to be uniformly continuous with respect to $W_p(D, D')$ for any $p$ with $1\leq p < \infty.$ (and indeed for all $p >0$.)  

Let $P_N(\Omega) $ be the set of all  persistence diagrams $D$ with $N$ data points; this is, those persistence diagrams $D$ of the form  $D= \{(x_n, y_n)\in \Omega:  1\leq n \leq N\}$.  Thus 
\begin{eqnarray}\label{0522.1}
P(\Omega) = \bigcup_{N=1}^\infty P_N(\Omega).
\end{eqnarray}
 Indeed the   $p$-Wasserstein distance $W_p(D, D')$ in 
\ref{0514.2} is  defined on 
\begin{eqnarray}\label{0524.6}
\bigcup_{N=1}^\infty P_N(\Omega)\times P_N(\Omega)
\end{eqnarray}

We now modify the proof of Proposition \ref{0512.A} to offer a uniform continuity analogue of the Proposition. 
 
%%%%%%%   Corollary   3.1      %%%%%%%%%%%


\begin{corollary}\label{0523.A} 
Suppose  $f: \Omega \to \R$ and $\la: \Omega \to (0, \infty)$ are bounded and uniformly continuous,  and $w:\Omega \to (0, \infty)$ is bounded. For any $N\geq 1$,  the  composite map $\tilde{f}\circ \rho :  P(\Omega) \to L^2(wdA)$ given by (\ref{0512.1})  is uniformly continuous  on $P_N(\Omega)$  with respect to $W_p(D, D')$ for any $p$ with $1\leq p < \infty.$ (and indeed for all $p >0$).
\end{corollary}


\begin{proof}
Let $M  > 0$ so that 
\begin{eqnarray}\label{0523.1}
 &   &  M \geq  \max\{|f(x,y)|:  (x, y) \in K\}, \ \mbox{and} \\ \label{0520.3}
 &  & M \geq  \max\{w(x,y):  (x, y) \in K\},  \ \mbox{and} \\ \label{0520.4}
 &   &  M \geq  \max\{\la(x,y):  (x, y) \in K\}.
\end{eqnarray}

Let  $\epsilon >0$. For the given integer $N$ in the statement of our corollary,  let 
\begin{eqnarray}\label{0522.2}
\delta_0 =  \frac{\epsilon}{\sqrt{32}N}.
\end{eqnarray}


Since $\la$ is uniform continuous on $\Omega$, there is a $\delta_1 >0$ such that 
\begin{eqnarray}\label{0522.3}
|\la(x,y) - \la(x', y')| <   \frac{\epsilon}{2M^{3/2}N},    \mbox{\ whenever}\  \|(x,  y) -  (x', y')\|_\infty \ < \ \delta_1.
\end{eqnarray}

Since $f$ is uniform continuous on $\Omega$,  there is a $\delta_2 >0$ such that 
\begin{eqnarray}\label{0524.3}
|f(x,y) -f(x', y')| <    \frac{\epsilon}{\sqrt{32} M^{3/2}N},   \mbox{\ whenever}\  \|(x, y) -  (x', y')\|_\infty \ < \ \delta_2.
\end{eqnarray}

Using $\delta_0, \delta_1, \delta_2$ defined above, let 
\begin{eqnarray}\label{0522.10}
\delta = \min\bigg(\delta_0, \delta_1, \delta_2, \frac{\epsilon^2}{16M^4N^2}\bigg)  >0.
\end{eqnarray}  
Suppose $D =\{(x_n, y_n): 1\leq n \leq N\}$ and $D' =\{(x_n', y_n'): 1\leq n \leq N\}$ are two persistence diagrams in $P_N(\Omega)$ with $W_p(D, D') < \delta.$  

Hence  by (\ref{0514.2})  there is a bijection $\sigma : \{1, 2, \ldots, N\} \to \{1, 2, \ldots, N\}$ such that 
\begin{eqnarray}\label{0522.4}
\sum_{n=1}^N \|(x_n, y_n)-(x_{\sigma(n)}', y_{\sigma(n)}') \|_\infty^p  \ < \ \delta^p,  \ \mbox{\ and hence}\\ \label{0522.5}
\|(x_n, y_n)-(x_{\sigma(n)}', y_{\sigma(n)}') \|_\infty  \ < \ \delta,  \ \mbox{ whenever }\ 1\leq n \leq N.  
\end{eqnarray}

By relabelling the points $(x_n', y_n')$ if necessary,  we assume without loss of generality that $\sigma(n) =n,$ for all $n$.   Thus we can rewrite (\ref{0522.5}) as
\begin{eqnarray}\label{0522.6} 
\|(x_n, y_n)-(x_n', y_n') \|_\infty  \ < \ \delta,  \ \mbox{ whenever }\ 1\leq n \leq N.  
\end{eqnarray}

To proceed further, we write $\la_n = \la(x_n, y_n)$ and $\la_n' = (x_n', y_n')$ and partition, according to Lemma \ref{0511.A},  the  set of integers in $\{1, 2, \ldots, N\}$,  into two subsets $A$ and $B$ given  by 
\begin{eqnarray}\label{0522.7}
A  & =  & \bigg\{n: 1\leq n \leq N,  \ \mbox{and} \ \|(x_n, y_n)-(x_n', y_n') \|_\infty  \ <  \ \frac{\la_n+\la_n'}{2}\bigg\}, \mbox{\ and}  \\ \label{0522.8}
B  & =  & \bigg\{n: 1\leq n \leq N,  \ \mbox{and} \ \|(x_n, y_n)-(x_n', y_n') \|_\infty  \ \geq \ \frac{\la_n+\la_n'}{2}\bigg\}
\end{eqnarray} 
 
 Thus we have 
\begin{eqnarray}\label{0523.2}
&  &  \|\tilde{f}(\rho(D) ) - \tilde{f}(\rho(D')) \| \\ \notag
& = & \bigg\| \sum_{n=1}^N f(x_n, y_n)\chi_{E_n} -  \sum_{n=1}^N f(x_n', y_n')\chi_{E_n'}\bigg\|  \\ \notag
& \leq & \sum_{n=1}^N \| f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}\| \\ \notag
& = & \sum_{n=1}^N \left( \int_\Omega| f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, wdA\right)^{1/2} \\ \notag
& = &  \bigg( \sum_{n\in A} \ + \ \sum_{n\in B} \bigg) \left( \int_\Omega | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, wdA\right)^{1/2}
\end{eqnarray}

We now focus on the above integral in two separate cases depending on whether the integer $n$ is in $A$ or in $B$. First if $n \in B$, then 
$\frac{\la_n+\la_n'}{2} \leq  \|(x_n, y_n)-(x_n', y_n') \|_\infty  < \delta$ and hence,  
$ \la_n< 2\delta$ and $ \la_n' < 2\delta.$

It follows from Statement (4) of Lemma \ref{0511.A} that if $n \in B$ then 
\begin{eqnarray}\label{0523.11}
&  & \int_\Omega | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, wdA  \ =  \  \la_n^2 + \la_n'^2 \\ \notag
&< & 4\delta^2 + 4\delta^2 \ = \  8 \delta^2\  < \ \frac{\epsilon^2}{4N^2}, \mbox{\ \  by (\ref{0522.10}) and (\ref{0522.2})}.
\end{eqnarray}
Hence we have 
\begin{eqnarray}\label{0522.11}
 \sum_{n\in B}  \left( \int_\Omega | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, wdA\right)^{1/2} \ \leq \ \sum_{n=1}^N  \sqrt{\frac{\epsilon^2}{4N^2}}  \ = \ \frac{\epsilon}{2}.
\end{eqnarray}

We now focus on the  integral in  (\ref{0523.2}) for $n \in A$. 
\begin{eqnarray}\label{0524.1}
& & \ \ \int_\Omega | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, wdA \\ \notag
&= & \ \ \int_{E_n \cup E_n'}\,  | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, wdA \\ \notag
&\leq& \  \ Mf(x_n, y_n)^2\, \mbox{Area}(E_n \setminus E_n') +  M (f(x_n, y_n) - f(x_n', y_n'))^2 \, \mbox{Area} (E_n \cap E_n') + \\ \notag
&   & + M f(x_n', y_n')^2 \mbox{Area} (E_n' \setminus E_n), \ \mbox{ by  (\ref{0520.3}).} \\ \notag
&\leq & \  M^3 \mbox{Area}(E_n \setminus E_n')  +  M (f(x_n, y_n) - f(x_n', y_n'))^2 \, \mbox{Area} (E_n \cap E_n') \\ \notag 
&  & +  M^3\mbox{Area}(E_n' \setminus E_n),  \ \mbox{ by  (\ref{0523.1}).}\\ \notag
\end{eqnarray}
We now use  Statement (3) of Lemma \ref{0511.A} and (\ref{0520.4}) to estimate Area$(E_n \setminus E_n')$ to get 
\begin{eqnarray}\label{0520.5}
{\rm Area}(E_n \setminus E_n')  \ \leq \   \la_n^2 - \bigg( \frac{\la_n+\la_n'}{2}\bigg)^2 + M|x- x'| +M|y-y'|,   \\ \notag
\end{eqnarray}
and by interchanging $E_n$ and $E_n'$ in (\ref{0520.5}),  we have 
\begin{eqnarray}\label{0520.6}
{\rm Area}(E_n' \setminus E_n) \  \leq  \   {\la_n'}^2 - \bigg( \frac{\la_n+\la_n'}{2}\bigg)^2 + M|x- x'| +M|y-y'|,   \\ \notag
\end{eqnarray}
Similarly using Statement (2) of Lemma \ref{0511.A} and (\ref{0520.4}) to estimate Area$(E_n \cap E_n')$, we get 
\begin{eqnarray}\label{0520.7}
{\rm Area}(E_n\cap E_n') \leq   (M-|x-x'|)(M-|y-y'|) \leq M^2.  \\ \notag
\end{eqnarray}


We now use the estimations in (\ref{0520.5}), (\ref{0520.6}), and (\ref{0520.7}) to continue our estimation in (\ref{0524.1}). We have that for $n\in A$, 
\begin{eqnarray}\label{0520.2} 
& & \ \ \int_\Omega | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, wdA \\ \notag
& \leq & M^3\left( \la_n^2 +{\la_n'}^2  - \left( \frac{\la_n + \la_n'}{2} \right)^2 \right)       \ + \ 2M^4\left(|x_n-x_n'| + |y_n-y_n'|\right) \ +  \ \\  \notag
& &  + M^3\left(f(x_n, y_n)  - f(x_n' - y_n')\right)^2.  \\ \notag
& = & M^3 \left( \frac{\la_n - \la_n'}{2} \right)^2       \ + \ 2M^4\left(|x_n-x_n'| + |y_n-y_n'|\right) \ +  \ M^3\left(f(x_n, y_n)  - f(x_n' - y_n')\right)^2.  
\end{eqnarray}

Hence, if $\|(x_n, y_n) - (x_n', y_n')\|_\infty < \delta,$ then we can use (\ref{0522.3}), (\ref{0524.3}), (\ref{0522.10}), and (\ref{0522.6}) to obtain 
\begin{eqnarray}\label{0524.4} 
& & \ \ \int_\Omega  | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, wdA \\ \notag
&\leq & M^3\frac{\epsilon^2}{16M^3N^2}      \ + \ 2M^4\frac{2\epsilon^2}{32M^4N^2} +  \ M^3\frac{\epsilon^2}{16M^3N^2}. \\ \notag
&=& \frac{\epsilon^2}{4N^2}.
\end{eqnarray} 

Therefore  we have 
\begin{eqnarray}\label{0524.5}
 \sum_{n\in A}  \left( \int_\Omega | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, wdA\right)^{1/2} 
\ \leq \ \sum_{n=1}^N  \sqrt{\frac{\epsilon^2}{4N^2}}  \ = \ \frac{\epsilon}{2}.
\end{eqnarray}

Putting our estimates in  (\ref{0524.5}) and  (\ref{0522.11}) into (\ref{0523.2}), we get that if $W_p(D, D') < \delta,$  
then 
\begin{eqnarray}\label{0524.7}
 \|\tilde{f}(\rho(D) ) - \tilde{f}(\rho(D')) \| \ < \ \frac{\epsilon}{2} +  \frac{\epsilon}{2} \ = \ \epsilon,
\end{eqnarray}
which finishes the proof for the uniform continuity of $\tilde{f}\circ \rho.$
\end{proof}

\bigskip 

%%%%%%%%%%   Remark 3.2   %%%%%%%%


\begin{remark}\label{0528.A} {\rm In the proof of the Proposition \ref{0523.A}, we have showed that for any positive $\epsilon,$ there is a positive $\delta >0$, given by (\ref{0522.10}), so that if (\ref{0522.4}) holds for $W_p(D, D')$, then (\ref{0524.7}) holds for $ \|\tilde{f}(\rho(D) ) - \tilde{f}(\rho(D')) \|$.  The formula 
 (\ref{0522.10}) for $\delta$ can help us determine {\bf discretization}  for our integration with respect to $wdA$.
}
\end{remark}

\bigskip


%%%%%%%%%  Example 3.3    %%%%%%%%%%%%

\begin{example}\label{0527.A} {\rm We now provide and example of a function $f(x, y)$  to show that the converse of Proposition \ref{0523.A}  does not hold.  Since every continuous   function  $f$ must be uniformly continuous on every compact subset of $\Omega$, we provide  an example of a function $f(x,y)$ that is not defined/not continuous on the $x$-axis.  Take $f(x, y) =  \sin(1/y)$, and  $\la(x, y) = \max(y, 1)$ and $\la(x,y) \equiv 1$.  Obviously $f$ is not uniformly continuous on the positive 
first quadrant.  We now prove that  $\tilde{f}\circ \rho :  P(\Omega) \to L^2(wdA)$ given by (\ref{0512.1})  is uniformly continuous  on $P_N(\Omega)$  
}\end{example}



\bigskip


\begin{proof} We follow the argument in the proof of Corollary \ref{0523.A} to prove the uniform continuity of $\tilde{f}\circ \rho$.   Let  $\epsilon >0$. For the given integer $N$ in the statement of our corollary,  let 
\begin{eqnarray}\label{0529.2}
\delta_0 =  \frac{\epsilon}{\sqrt{32}N}.
\end{eqnarray}




Since $f$ is  uniformly continuous on $\{ (x, y) \in \Omega:   y \geq \delta_0 \}$,  there is a $\delta_1 >0$ such that whenever $(x, y) \in \Omega$ with $y, y'\geq \delta_0$ with $|y-y'| < \ \delta_1,$
\begin{eqnarray}\label{0529.5}
|f(x,y) -f(x', y')| \  < \  \bigg|\sin\frac{1}{y} - \sin\frac{1}{y'}\bigg| \  <  \ \frac{\epsilon}{\sqrt{12}N}  
\end{eqnarray}

Since $\la$ is uniformly continuous on $\Omega$, there is a $\delta_2 > 0$ such that whenever $(x, y) \in \Omega$ with  $|y-y'| < \ \delta_2,$
\begin{eqnarray}\label{0529.25}
|\la(x,y) -\la(x', y')| \  <   \ \frac{\epsilon}{\sqrt{3}N}  
\end{eqnarray}


Using $\delta_0, \delta_1, \delta_2$ defined above, let 
\begin{eqnarray}\label{0529.8}
\delta = \min\bigg(\delta_0, \delta_1, \delta_2, \frac{\epsilon^2}{48N^2}\bigg)  >0.
\end{eqnarray}  
Suppose $D =\{(x_n, y_n): 1\leq n \leq N\}$ and $D' =\{(x_n', y_n'): 1\leq n \leq N\}$ are two persistence diagrams in $P_N(\Omega)$ with $W_p(D, D') < \delta.$  

Hence  by (\ref{0514.2})  there is a bijection $\sigma : \{1, 2, \ldots, N\} \to \{1, 2, \ldots, N\}$ such that 
\begin{eqnarray}\label{0529.4}
\sum_{n=1}^N \|(x_n, y_n)-(x_{\sigma(n)}', y_{\sigma(n)}') \|_\infty^p  \ < \ \delta^p,  \ \mbox{\ and hence}\\ \label{0529.20}
\|(x_n, y_n)-(x_{\sigma(n)}', y_{\sigma(n)}') \|_\infty  \ < \ \delta,  \ \mbox{ whenever }\ 1\leq n \leq N.  
\end{eqnarray}

By relabelling the points $(x_n', y_n')$ if necessary,  we assume without loss of generality that $\sigma(n) =n,$ for all $n$.   Thus we can rewrite (\ref{0529.20}) as
\begin{eqnarray}\label{0529.6} 
\|(x_n, y_n)-(x_n', y_n') \|_\infty  \ < \ \delta,  \ \mbox{ whenever }\ 1\leq n \leq N.  
\end{eqnarray}

To proceed further, we write $\la_n = \la(x_n, y_n) $ and $\la_n' = (x_n', y_n')'$ and partition, according to Lemma \ref{0511.A},  the  set of integers in $\{1, 2, \ldots, N\}$,  into two subsets $A$ and $B$ given  by 
\begin{eqnarray}\label{0529.7}
A  & =  & \bigg\{n: 1\leq n \leq N,  \ \mbox{and} \ \|(x_n, y_n)-(x_n', y_n') \|_\infty  \ <  \ \frac{\la_n+\la_n'}{2}\bigg\}, \mbox{\ and}  \\ \label{0529.0}
B  & =  & \bigg\{n: 1\leq n \leq N,  \ \mbox{and} \ \|(x_n, y_n)-(x_n', y_n') \|_\infty  \ \geq \ \frac{\la_n+\la_n'}{2}\bigg\}
\end{eqnarray} 
 
 Thus we have 
\begin{eqnarray}\label{0529.9}
&  &  \|\tilde{f}(\rho(D) ) - \tilde{f}(\rho(D')) \| \\ \notag
& = & \bigg\| \sum_{n=1}^N f(x_n, y_n)\chi_{E_n} -  \sum_{n=1}^N f(x_n', y_n')\chi_{E_n'}\bigg\|  \\ \notag
& \leq & \sum_{n=1}^N \| f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}\| \\ \notag
& = & \sum_{n=1}^N \left( \int_\Omega| f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, wdA\right)^{1/2} \\ \notag
& = &  \bigg( \sum_{n\in A} \ + \ \sum_{n\in B} \bigg) \left( \int_\Omega | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, dA\right)^{1/2}
\end{eqnarray}

We now focus  on the above integral in two separate cases depending on whether the integer $n$ is in $A$ or in $B$. First if $n \in B$, then 
$ \frac{\la_n+\la_n'}{2} \leq  \|(x_n, y_n)-(x_n', y_n') \|_\infty  < \delta$ and hence,  
$\la_n< 2\delta$ and $ \la_n' < 2\delta.$

It follows from Statement (4) of Lemma \ref{0511.A} that if $n \in B$ then 
\begin{eqnarray}\label{0529.10}
&  & \int_\Omega | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, dA  \ =  \  \la_n^2 + \la_n'^2 \\ \notag
&< & 4\delta^2 + 4\delta^2 \ = \  8 \delta^2\  < \ \frac{\epsilon^2}{4N^2}, \mbox{\ \  by (\ref{0529.2}) and (\ref{0529.8})}.
\end{eqnarray}
Hence we have 
\begin{eqnarray}\label{0529.11}
 \sum_{n\in B}  \left( \int_\Omega | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, dA\right)^{1/2} \ \leq \ \sum_{n=1}^N  \sqrt{\frac{\epsilon^2}{4N^2}}  \ = \ \frac{\epsilon}{2}.
\end{eqnarray}


We now focus on the  integral in  (\ref{0529.9}) for $n \in A$. 
\begin{eqnarray}\label{0529.12}
& & \ \ \int_\Omega | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, dA \\ \notag
&= & \ \ \int_{E_n \cup E_n'}\,  | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, dA \\ \notag
&\leq& \  \ f(x_n, y_n)^2\, \mbox{Area}(E_n \setminus E_n') +  (f(x_n, y_n) - f(x_n', y_n'))^2 \, \mbox{Area} (E_n \cap E_n') + \\ \notag
&   & +  f(x_n', y_n')^2 \mbox{Area} (E_n' \setminus E_n), \\ \notag
&\leq & \   \mbox{Area}(E_n \setminus E_n')  +   (f(x_n, y_n) - f(x_n', y_n'))^2 \, \mbox{Area} (E_n \cap E_n') \\ \notag 
&  & +  \mbox{Area}(E_n' \setminus E_n).  \\ \notag
\end{eqnarray}

We now estimate Area$(E_n \setminus E_n')$, using  Statement (3) of Lemma \ref{0511.A} and our choice of $\la$ given by $\la(x,y) = \max(y, 1)$.  
\begin{eqnarray}\label{0529.13}
{\rm Area}(E_n \setminus E_n')  \ \leq \   \la_n^2 - \bigg( \frac{\la_n+\la_n'}{2}\bigg)^2 + |x- x'| +|y-y'|,   \\ \notag
\end{eqnarray}
and by interchanging $E_n$ and $E_n'$ in (\ref{0529.13}),  we have 
\begin{eqnarray}\label{0529.14}
{\rm Area}(E_n' \setminus E_n) \  \leq  \   {\la_n'}^2 - \bigg( \frac{\la_n+\la_n'}{2}\bigg)^2 + |x- x'| +|y-y'|,   \\ \notag
\end{eqnarray}
Similarly using Statement (2) of Lemma \ref{0511.A} to estimate Area$(E_n \cap E_n')$, we get 
\begin{eqnarray}\label{0529.15}
{\rm Area}(E_n\cap E_n') \leq   (1-|x-x'|)(1-|y-y'|) \leq 1.  \\ \notag
\end{eqnarray}



We now use the estimations in (\ref{0529.13}), (\ref{0529.14}), and (\ref{0529.15}) to continue our estimation in (\ref{0529.12}). We have that for $n\in A$, 
\begin{eqnarray}\label{0529.16} 
& & \ \ \int_\Omega | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, dA \\ \notag
& \leq & \left( \la_n^2 +{\la_n'}^2  - \left( \frac{\la_n + \la_n'}{2} \right)^2 \right)       \ + \ 2\left(|x_n-x_n'| + |y_n-y_n'|\right) \ +  \ \\  \notag
& &  + \left(f(x_n, y_n)  - f(x_n' - y_n')\right)^2.  \\ \notag
& = &  \left( \frac{\la_n - \la_n'}{2} \right)^2       \ + \ 2\left(|x_n-x_n'| + |y_n-y_n'|\right) \ +  \ \left(f(x_n, y_n)  - f(x_n' - y_n')\right)^2.  
\end{eqnarray}

Hence, if $\|(x_n, y_n) - (x_n', y_n')\|_\infty < \delta,$ then we can use (\ref{0529.8}), (\ref{0529.25}), (\ref{0529.5}) on our estimate in (\ref{0529.16})  to obtain 
\begin{eqnarray}\label{0529.17} 
& & \ \ \int_\Omega  | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, dA \\ \notag
&\leq &  \frac{1}{4} \bigg(\frac{\epsilon^2}{3N^2} \bigg)  \ + \ 4\delta +  \frac{\epsilon^2}{12N^2} \\ \notag
&\leq & \frac{\epsilon^2}{12N^2}  + 4\bigg( \frac{\epsilon^2}{48N^2} \bigg) +  \frac{\epsilon^2}{12N^2},   \mbox{ by (\ref{0529.8})}\\ \notag
&=& \frac{\epsilon^2}{4N^2}. 
\end{eqnarray} 

Therefore  we have 
\begin{eqnarray}\label{0529.18}
 \sum_{n\in A}  \left( \int_\Omega | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, dA\right)^{1/2} 
\ \leq \ \sum_{n=1}^N  \sqrt{\frac{\epsilon^2}{4N^2}}  \ = \ \frac{\epsilon}{2}.
\end{eqnarray}

Putting our estimates in  (\ref{0529.11}) and  (\ref{0529.18}) into (\ref{0529.9}), we get that if $W_p(D, D') < \delta,$  
then 
\begin{eqnarray}\label{0529.19}
 \|\tilde{f}(\rho(D) ) - \tilde{f}(\rho(D')) \| \ < \ \frac{\epsilon}{2} +  \frac{\epsilon}{2} \ = \ \epsilon,
\end{eqnarray}
which finishes the proof for the uniform continuity of $\tilde{f}\circ \rho.$
\end{proof}




{\bf Conjecture 3A:}   The following statements are equivalent:
\begin{enumerate}
\item[(1) ] $\tilde{f}\circ \rho$ is continuous  on $P_N(\Omega)$ with respect to $W_p(D, D')$ for some $N \geq 1$ and some $p$ with $0 \leq p < \infty.$
\item[(2)] $\tilde{f}\circ \rho$ is continuous  on $P_N(\Omega)$ with respect to $W_p(D, D')$ for all  $N \geq 1$ and some $p$ with $0 \leq p < \infty.$
\item[(3)] $\tilde{f}\circ \rho$ is continuous  on $P_N(\Omega)$ with respect to $W_p(D, D')$ for some  $N \geq 1$ and all $p$ with $0 \leq p < \infty.$
\item[(4)] $\tilde{f}\circ \rho$ is continuous  on $P_N(\Omega)$ with respect to $W_p(D, D')$ for all  $N \geq 1$ and all $p$ with $0 \leq p < \infty.$
\end{enumerate}

Remark: Of course, it suffices to show Statements (1) and (4) are equivalent.

\bigskip 

{\bf Conjecture 3B:}   Replace the word "continuous" by "uniformly continuous" in Conjecture 3A. 

\bigskip


{\bf Conjecture 3C:}   instead of using the sup-norm $\|\cdot \|_\infty$ to define  $W_p(D, D')$ in 
(\ref{0514.2})  on 
\begin{eqnarray}\label{0526.1}
\bigcup_{N=1}^\infty P_N(\Omega)\times P_N(\Omega),
\end{eqnarray}
we can use the $p$-norm $\|\cdot\|_p$. 
That is,  $W_p(D, D')$ can be defined by 
\begin{eqnarray}\label{0526.2}
&  & W_p(D, D') \\  \notag
&= &  \inf\bigg\{ \bigg( \sum_{n=1}^N \|(x_n\,  y_n) -  (x_{\sigma(n)}', y_{\sigma(n) }')\|_p^p \bigg)^{1/p} \, \bigg|\,  \sigma \text{ is a bijection on } \{1, 2, \ldots N\} \bigg\}.
\end{eqnarray}
on $\bigcup P_N(\Omega)\times P_N(\Omega).$
Since each $P_N(\Omega)$ is  finite dimensional, any two norms are equivalent, and in particular the sup-norm $\|\cdot \|_\infty$ and the $p$-norm
$\|\cdot \|_p$.  So, if $N$ is fixed, the two $W_p(D, D')$ defined by (\ref{0514.2})  and (\ref{0526.2}) are equivalent. 



\bigskip

{\bf Problem 3D:}  Prove the converse of Proposition \ref{0523.A}. Or provide a condition so that if $\tilde{f}\circ \rho$ is uniformly continuous then $f$ is uniformly continuous.  

\bigskip


{\bf Problem 3E:} We have to give four examples to show that each of the hypotheses  on $\la$ and $w$ in Proposition \ref{0523.A} and  Problem 3D  are  necessary for the two propositions to hold.
\end{subsection}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%         SECTION 4        %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{subsection}{June 1, 2020}\label{1June2020}

{\bf  NOTE THAT WE HAVE CHANGED THE DEFINITION FOR $W_{1/2}(D, D')$ IN THIS SECTION FROM THE PREVIOUS SECTIONS}

In this section, we are trying to establish the analogue of \cite[3rd Inequality, Theorem 5, page 11]{AEKNP}.  Following our notation and set up in Section \ref{17May2020}, we  continue to use   $P(\Omega)$  to denote  the collection of all persistence diagrams $D = \{(x_n, y_n) \in \Omega:  1 \leq n \leq N\}$ where $N \geq 1$ is an integer. We continue to use the symbol  $\rho$ as defined in (\ref{0513.1}). The symbol $\tilde{f}(\rho (D))$ defined by (\ref{0512.1}) is called the persistence surface in \cite[Definition 1, page 8]{AEKNP}, and the symbol $W_p(D, D')$ defined by (\ref{0514.2}) is the $p$-Wasserstein distance $W_p(D, D')$ in \cite[line -5, page 7]{AEKNP}. 

As in the beginning of Section \ref{26May2020}, we let $P_N(\Omega) $ be the set of all  persistence diagrams $D$ with $N$ data points; this is, those persistence diagrams $D$ of the form  $D= \{(x_n, y_n)\in \Omega:  1\leq n \leq N\}$. 
 
 %%%%%%%% Lemma 4.1  %%%%%%
 
 
 
 We repeat the following from  a previous section here:
 \begin{lemma}\label{0511.AA}
Let  $E$ and $E'$ be two squares  with same side lengths $\la$ and $\la'$, centered at $(x, y)$ and $(x', y')$ respectively. We have the following Statements. 
\begin{enumerate}
\item[(1)] {\rm Area}$(E\cap E') > 0 $ if and only if $\displaystyle{ \|(x, y) - (x', y')) \|_\infty \  <  \ \frac{\la+\la'}{2};}$   
\item[(2)] If {\rm Area}$(E\cap E') > 0 $, then $${\rm Area}(E\cap E')  = \bigg( \frac{\la+\la'}{2}-|x-x'|\bigg)\bigg( \frac{\la+\la'}{2}-|y-y'|\bigg);$$
  \ \item[(3)]  If {\rm Area}$(E\cap E') > 0 $, then  
  \begin{eqnarray}\notag
  &   & {\rm Area}(E\setminus E') \\ \notag
&  = &  \la^2  -  {\rm Area} (E\cap E') \\ \notag
 & = &  \la^2-  \bigg( \frac{\la+\la'}{2}-|x-x'|\bigg)\bigg( \frac{\la+\la'}{2}-|y-y'|\bigg) \\ \notag
 & = & \la^2 - \bigg( \frac{\la+\la'}{2}\bigg)^2 + \bigg( \frac{\la+\la'}{2}\bigg)|x- x'| + \bigg( \frac{\la+\la'}{2}\bigg)|y-y'|    - |x-x'|\, |y-y'|. 
 \end{eqnarray}
 \item[(4)] {\rm Area}$(E\cup E') = \la^2+ {\la'}^2$ when  $\displaystyle{ \|(x, y) - (x', y')) \|_\infty \ \geq \  \frac{\la+\la'}{2}.}$
\end{enumerate} 
\end{lemma} 

 In \cite[Definition 2, page 8]{AEKNP}, as well as \cite[line -5, page 11]{AEKNP}, a pixel is denoted by $p$, which is the same symbol $p$ is also used 
 in $W_p(D, D')$, and so we used $S$ to denote a pixel (which we picture as a small square $S$). 
  Suppose all vectors $\tilde{f}\circ \rho(D)$ of  persistence diagrams $D$ are contained in a region, on which $\mathcal P$ is the partition of that region  into  pixels $S$. 

The following  definition is from  \cite[Definition 2, page 8]{AEKNP}, with a slight change of notation here; see also  \cite[first sentence, Theorem 5, page 11]{AEKNP}.
\begin{definition}\label{0604.A}
{\rm The} \mbox{ persistence image} $I(D)$ {\rm  of a persistence diagram} D {\rm is the collection of} \ $\displaystyle{I_S(D) = \int_S \tilde{f}\circ \rho(D) wdA,}$ {\rm where} $S\in \mathcal P$. 
\end{definition}

The following definition is used implicitly in the proof of   \cite[Theorem 5, page 11]{AEKNP}. We define a $p$-norm on all persistence images by 
\begin{definition}\label{0604.B}
$\displaystyle{  \|I(D) - I(D')\|_p \ = \  \bigg( \sum_{S\in \mathcal P} | I_S(D) - I_S(D') |^p \bigg)^{1/p},}$  {\rm for} $1\leq p < \infty.$
\end{definition}

Correspondingly the sup-norm is given by 
\begin{definition}\label{0604.C}
$\displaystyle{  \|I(D) - I(D')\|_\infty \ = \ \sup_{S\in \mathcal P} | I_S(D) - I_S(D') | }$
\end{definition}

In the following lemma, we use the notation  $d\mu = wdA$. That is, for any Lebesgue measurable set $E$,
$$\mu (E) \ = \ \int_E \, d\mu \ = \ \int_E\, wdA.$$


%%%%%%%%%    Lemma 4.5   %%%%%%%%%

\begin{lemma}\label{0604.D}   
Let $D = \{(x_n, y_n): 1\leq n \leq N\}$ and $D' = \{(x_n', y_n'): 1\leq n \leq N\}$.  Using the notation $d\mu = wdA$, we have for $p =2$ in Definition \ref{0604.B}, 
\begin{eqnarray}\label{0605.1}
&  &  \| I(D) - I(D')\|^2_2 \\ \notag
&\leq &  \sum_{S\in \mathcal P} \mu(S) \left( \sum_{1\leq n\leq N} \left( \int_S |f(x_n, y_n) \chi_{E_n} - f(x_n', y_n')\chi_{E_n'}|^2 \, wdA\right)^{\frac{1}{2}} \right)^2.
 \end{eqnarray}
\end{lemma}

\begin{proof}  For any pixel S in $\mathcal P$, 
\begin{eqnarray}\label{0604.1}
&  &  |I_S(D) - I_S(D')|^2   \\ \notag
& = &  \bigg( \int_S\tilde{f}\circ \rho(D) \,wdA - \int_S\tilde{f}\circ \rho(D') wdA \bigg)^2 \\ \notag
& \leq &  \bigg( \int_S | \tilde{f}\circ \rho(D) - \tilde{f}\circ \rho(D') |  wdA \bigg)^2 \\ \notag
& \leq &  \bigg( \int_S | \tilde{f}\circ \rho(D) - \tilde{f}\circ \rho(D') |^2  wdA \bigg)\bigg( \int_S 1^2\, wdA \bigg),  \mbox{by the Cauchy-Schwarz inequality}  \\ \notag
& \leq & \mu(S) \bigg( \int_S | \tilde{f}\circ \rho(D) - \tilde{f}\circ \rho(D') |^2  wdA \bigg) 
\end{eqnarray}

If we let  $\|\cdot\|_S$ be the Hilbert norm given by 
\begin{eqnarray}\label{0604.2}
\| g \|_s = \bigg( \int_S |g|^2 wdA \bigg)^{1/2}, 
\end{eqnarray}
then we can continue we estimation in  \ref{0604.1} as follows. 
\begin{eqnarray}\label{0604.3}
&  &  |I_S(D) - I_S(D')|^2   \\ \notag
& \leq & \mu(S) \| \tilde{f}\circ \rho(D) - \tilde{f}\circ \rho(D') \|_S^2  \\ \notag
& \leq & \mu(S) \bigg(  \sum_{1\leq n \leq N} \, \| f(x_n, y_n)\chi_{E_n} - f(x_n', y_n')\chi_{E_n'} \|_S  \bigg)^2, \mbox{ by the triangle inequality}  \\ \notag
& = & \mu(S) \left(  \sum_{1\leq n \leq N} \, \left( \int_S | f(x_n, y_n)\chi_{E_n} - f(x_n', y_n')\chi_{E_n'}|^2 \, wdA \right)^{\frac{1}{2}} \right)^2.
\end{eqnarray}
Taking the sum over all pixels $S$ in $\mathcal P$, we finish the proof.
\end{proof} 
 


In the following proposition, we define for two persistence diagrams $D, D'$  in $P_N(\Omega)$, 
\begin{eqnarray}\label{0605.5}
&  & W_{1/2}(D, D') \\ \notag
&= &  \inf \left\{  \sum_{n=1}^N \|(x_n\,  y_n) -  (x_{\sigma(n)}', y_{\sigma(n) }')\|_\infty^{1/2} \, :  \, \sigma \text{ is a bijection on } \left\{1, 2, \ldots, N\right\}\right\}.
\end{eqnarray}
{\bf Remark:} We do NOT take the square over the sum in the above definition, because the sum itself defines a metric (but not a norm) on the sequence space $\ell^{1/2}$. 

% %   Proposition 4.6 

\begin{proposition}\label{0601.A} 
Let $\mathcal P$ be a collection of pixels $S$ whose union $\Omega_0$ contains 
$\rho(D)$ and $\rho(D')$.
 Suppose  $f: \Omega \to \R$ and $\la: \Omega \to (0, \infty)$ are bounded and  Lipchitz with positive  constants $C_f$ and $C_\la$ respectively: 
\begin{eqnarray}\label{0601.100}
|f(x, y) - f(x',y')| \ \leq \ C_f \|((x, y) - (x', y')\|_\infty \\ \label{0601.200}
|\la(x, y) - \la(x',y')| \ \leq \ C_\la \|((x, y) - (x', y')\|_\infty
\end{eqnarray}
Let $w:\Omega \to (0, \infty)$ is bounded with $0 < w(x, y) \leq M$ for all $(x, y) \in \Omega$.   If  $C_2>0$ is a constant given by 
\begin{eqnarray}\label{0605.2}
C_2^2 = M^2\|f\|_\infty \|\la\|_\infty \max\{4\|f\|_\infty, \ (C_\la +  4)\|f\|_\infty + 2 C_f \|\la\|_\infty\},
\end{eqnarray}
then we have 
\begin{eqnarray}\label{0601.400}
\| I(D) - I(D') \|_2   \leq   C_2 \sqrt{{\rm Area}(\Omega_0) }\,W_{1/2}(D, D').
\end{eqnarray}

\end{proposition}

{\bf Remark.} When compared with \cite[third inequality, Theorem 5, page 11]{AEKNP}, our inequality (\ref{0601.400}) has advantage that it does not 
depend on the number of pixels in $\Omega_0$.   However, in the case that each pixel has the exact same area $A$, then the term $\sqrt{n}A$ can be interpreted as  $\sqrt{A}\sqrt{{\rm Area}(\Omega_0)}$, which is essentially what we have in Proposition (\ref{0601.400}).


\begin{proof} Suppose $D =\{(x_n, y_n): 1\leq n \leq N\}$ and $D' =\{(x_n', y_n'): 1\leq n \leq N\}$ are two persistence diagrams in $P_N(\Omega)$. 
Let  $\sigma : \{1, 2, \ldots, N\} \to \{1, 2, \ldots, N\}$  be a bijection such that 
\begin{eqnarray}\label{0602.1}
W_{1/2} (D, D') =  \sum_{n=1}^N \|(x_n\,  y_n) -  (x_{\sigma(n)}', y_{\sigma(n) }')\|_\infty^{1/2}
\end{eqnarray}

By relabelling the points $(x_n', y_n')$ if necessary,  we assume without loss of generality that $\sigma(n) =n,$ for all $n$.   Thus we can rewrite (\ref{0602.1}) as
\begin{eqnarray}\label{0602.2}
W_{1/2}(D, D') =   \sum_{n=1}^N \|(x_n\,  y_n) -  (x_n', y_n')\|_\infty^{1/2}. 
\end{eqnarray}

To proceed further, we write $\la_n = \la(x_n, y_n) $ and $\la_n' = (x_n', y_n')$ and partition, according to Lemma \ref{0511.AA},  the  set of integers in $\{1, 2, \ldots, N\}$,  into two subsets $A$ and $B$ given  by 
\begin{eqnarray}\label{0601.7}
A  & =  & \bigg\{n: 1\leq n \leq N,  \ \mbox{and} \ \|(x_n, y_n)-(x_n', y_n') \|_\infty  \ <  \ \frac{\la_n+\la_n'}{2}\bigg\}, \mbox{\ and}  \\ \label{0601.0}
B  & =  & \bigg\{n: 1\leq n \leq N,  \ \mbox{and} \ \|(x_n, y_n)-(x_n', y_n') \|_\infty  \ \geq \ \frac{\la_n+\la_n'}{2}\bigg\}
\end{eqnarray} 


 
We now use Lemma \ref{0604.D} to prove our Proposition, by 
considering the integral  in  
(\ref{0605.1}) in two different ways, depending on whether the integer $n$ is in $A$ or in $B$. First if $n \in B$  then 
$ \frac{\la_n+\la_n'}{2} \leq  \|(x_n, y_n)-(x_n', y_n') \|_\infty,$ and hence
\begin{eqnarray}\label{0602.3} 
 \la_n< 2\|(x_n, y_n)-(x_n', y_n') \|_\infty,  \mbox{  and  }\  \la_n' < 2\|(x_n, y_n)-(x_n', y_n') \|_\infty. 
\end{eqnarray}
Thus if $n \in B$ then by Statement (1) of Lemma \ref{0511.AA}, we have $E_n \cap E_n' = \emptyset$, and so for a  pixel $S$, we have 
\begin{eqnarray}\label{0601.10}
&   &  \int_S | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, wdA  \\ \label{0602.5}
& \leq  &  M\|f\|_\infty^2 \mbox{Area}(E_n ) + M \|f\|_\infty^2 \mbox{Area}(E_n')  \\ \label{0602.6}
& \leq &  M\|f\|_\infty^2 \la_n^2+ M \|f\|_\infty^2 {\la'}_n^2  \\ \label{0602.7}
& \leq &  M\|f\|_\infty^2 \|\la\|_\infty \la_n+ M \|f\|_\infty^2   \|\la\|_\infty {\la'}_n  \\ \label{0602.71}
& < & 4M\|f\|_\infty^2  \|\la\|_\infty \|(x_n, y_n)-(x_n', y_n') \|_\infty, \mbox{\ by (\ref{0602.3}).} 
\end{eqnarray}





Second, we  now focus on the integers $n \in A$, for which we use Statement (1) of Lemma \ref{0511.AA} to obtain 
\begin{eqnarray}\label{0601.12}
& & \ \ \int_S | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, wdA \\ \label{0602.8}
&\leq & \ \ \int_{(E_n \cup E_n')\cap S}\, M | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, dA \\ \label{0602.9}
&\leq& \  \ M|f(x_n, y_n)|^2\mbox{Area}\left((E_n \setminus E_n')\cap S\right) +  M| f(x_n', y_n')|^2 \mbox{Area} \left((E_n' \setminus E_n)\cap S\right) + \\ \notag
&   & + M |f(x_n, y_n) - f(x_n', y_n')|^2 \, \mbox{Area} \left((E_n \cap E_n')\cap S\right) \\ \label{0602.10}
&\leq&  \ \ M\|f\|_\infty^2 \bigg( \mbox{Area}\left((E_n \setminus E_n')\cap S\right)  +  \mbox{Area} \left((E_n' \setminus E_n)\cap S\right) \bigg) + \\ \notag&   & + 2M\|f\|_\infty |f(x_n, y_n) - f(x_n', y_n')| \, \mbox{Area} \left((E_n \cap E_n')\cap S\right) \\ \label{0602.10.1}
&\leq & \ \ M\|f\|_\infty^2 \bigg( \mbox{Area}\left((E_n \setminus E_n')\cap S\right)  +  \mbox{Area} \left((E_n' \setminus E_n)\cap S\right) \bigg) + \\ \notag
&   & + 2M \|f\|_\infty C_f \|((x_n, y_n) - (x_n', y_n')\|_\infty \, \mbox{Area} (E_n), \mbox{ \ by (\ref{0601.100})}.
\end{eqnarray}


We now estimate the term $ \mbox{Area}\left((E_n \setminus E_n')\cap S\right)  +  \mbox{Area} \left((E_n' \setminus E_n)\cap S\right)$  in (\ref{0602.10.1}), using Statement (3) of Lemma \ref{0511.AA}.
First, 
\begin{eqnarray}\label{0601.13}
&  & \mbox{Area}\left((E_n \setminus E_n')\cap S\right) \  \leq \  {\rm Area}(E_n \setminus E_n')   \\ \notag
& \leq &    \la_n^2 - \bigg( \frac{\la_n+\la_n'}{2}\bigg)^2 + \|\la\|_\infty ( |x_n- x_n'| +|y_n-y_n'|), 
\end{eqnarray}
and by interchanging $E_n$ and $E_n'$ in (\ref{0601.13}), then we have 
\begin{eqnarray}\label{0601.14}
& &  \mbox{Area} \left((E_n' \setminus E_n)\cap S\right) \ \leq \ {\rm Area}(E_n' \setminus E_n)   \\ \notag
& \leq &     {\la_n'}^2 - \bigg( \frac{\la_n+\la_n'}{2}\bigg)^2 + \|\la\|_\infty ( |x_n- x_n'| +|y_n-y_n'|). 
\end{eqnarray}
By summing (\ref{0601.13}) and (\ref{0601.14}) we have 
\begin{eqnarray}\label{0601.15}
&  & \mbox{Area}\left((E_n \setminus E_n')\cap S\right)  +  \mbox{Area} \left((E_n' \setminus E_n)\cap S\right)  \\ \notag
&\leq &   \la_n^2  + { \la_n'}^2 - 2 \bigg( \frac{\la_n+\la_n'}{2}\bigg)^2 + 2\|\la\|_\infty ( |x_n- x_n'| +|y_n-y_n'|) \\ \notag
& = &  \bigg( \frac{\la_n- \la_n'}{2}\bigg)^2 + 2\|\la\|_\infty ( |x_n- x_n'| +|y_n-y_n'|) \\ \notag
& = &\bigg( \frac{ \|\la\|_\infty + \|\la\|_\infty}{2}\bigg) \bigg( \frac{\la_n- \la_n'}{2}\bigg) + 2\|\la\|_\infty ( |x_n- x_n'| +|y_n-y_n'|) \\ \notag
& \leq & \|\la\|_\infty \frac{C_\la}{2} \|((x_n, y_n) - (x_n', y_n')\|_\infty +  4\|\la\|_\infty  \|((x_n, y_n) - (x_n', y_n')\|_\infty, \mbox{ \ by (\ref{0601.200})}. \\ \notag
&\leq &  \|\la\|_\infty (C_\la +  4) \|((x_n, y_n) - (x_n', y_n')\|_\infty
\end{eqnarray}




Using (\ref{0601.15})  to continue our estimations in (\ref{0602.10.1}), we get that if $n\in A$ then 
\begin{eqnarray}\label{0602.12}
& & \ \ \int_S | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, wdA \\  \notag
&\leq &  \ \ M\|f\|_\infty^2 \|\la\|_\infty (C_\la +  4) \|((x_n, y_n) - (x_n', y_n')\|_\infty + \\  \notag
&   & + 2M \|f\|_\infty C_f  \|\la\|_\infty^2\|((x_n, y_n) - (x_n', y_n')\|_\infty.\\ \notag
&\leq & \bigg( M(C_\la +  4)\|f\|_\infty^2 \|\la\|_\infty + + 2M C_f \|f\|_\infty \|\la\|_\infty^2\bigg)  \|((x_n, y_n) - (x_n', y_n')\|_\infty 
\end{eqnarray}


It follows from (\ref {0601.10}) and  (\ref{0602.12}) that if we let $C_2$ be given by (\ref{0605.2}), then for all integers $n$ with $1\leq n \leq N$, we have 
\begin{eqnarray}\label{0605.3}
& & \ \ \int_S | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}|^2 \, wdA \ \leq \         \frac{C_2^2}{M}\|((x_n, y_n) - (x_n', y_n')\|_\infty 
\end{eqnarray}

We now use Lemma \ref{0604.D} to conclude that 
\begin{eqnarray}\label{0605.4}
&  &  \| I(D) - I(D')\|^2_2 \\ \notag
&\leq &  \sum_{S\in \mathcal P} \mu(S) \left( \sum_{1\leq n\leq N} \left( \frac{C_2^2}{M}\|((x_n, y_n) - (x_n', y_n')\|_\infty \right)^{\frac{1}{2}} \right)^2. \\ \notag
&\leq &  \frac{C_2^2}{M} W_{1/2}(D, D')^2 \sum_{S\in \mathcal P} \mu(S). \\ \notag
&=  &  \frac{C_2^2}{M} W_{1/2}(D, D')^2 \mu(\Omega_0). \\ \notag
&\leq &  \frac{C_2^2}{M}M  \mbox{Area}(\Omega_0) W_{1/2}(D, D')^2. \\ \notag
&\leq & {C_2^2}  \mbox{Area}(\Omega_0) W_{1/2}(D, D')^2,
 \end{eqnarray}
 which finishes our proof.
 \end{proof}
 
 
 %%%%%%%   Corollary 4.7    %%%%%%%
 
 \begin{corollary}\label{0605.B}
With the  same hypotheses  in Proposition \ref{0601.A}, we have 
\begin{eqnarray}\label{0605.6}
\| I(D) - I(D') \|_1   \leq  \bigg( \frac{C_2}{\sqrt M} \sum_{S\in \mathcal P} \sqrt{\mu(S)} \bigg) W_{1/2}(D, D').
\end{eqnarray}
 \end{corollary}


\begin{proof}  By Definition \ref{0604.B}, we have 
\begin{eqnarray}\label{0605.7}
&   &   \|I(D) - I(D')\|_1 \\ \notag
 & = &  \sum_{S\in \mathcal P} | I_S(D) - I_S(D') | \\ \notag
& \leq &\sum_{S\in \mathcal P}  \sqrt{ \mu(S)} \sum_{1\leq n \leq N} \, \left( \int_S | f(x_n, y_n)\chi_{E_n} - f(x_n', y_n')\chi_{E_n'}|^2 \, wdA \right)^{\frac{1}{2}}, \mbox{by (\ref{0604.3})}\\ \notag
& \leq &\sum_{S\in \mathcal P}  \sqrt{ \mu(S)} \sum_{1\leq n \leq N} \, \left( \frac{C_2^2}{M}\|((x_n, y_n) - (x_n', y_n')\|_\infty  \right)^{\frac{1}{2}}, \ \mbox{by (\ref{0605.3})}.  
\end{eqnarray}
\end{proof} 


%%%%%%   Proposition 4.8   %%%%%%

\begin{proposition}\label{0605.C} 
With the same hypotheses in Proposition \ref{0601.A}, let $C_1>0$ be given by 
\begin{eqnarray}\label{0605.20}
C_1 = M \|\la\|_\infty\, \max\{ 4\|f\|_\infty ,   \  \|f\|_\infty (C_\la +  4) +  C_f \|\la\|_\infty\}. 
\end{eqnarray}
Then we have 
\begin{eqnarray}\label{0605.14}
\| I(D) - I(D') \|_1  \leq  C_1 W_1(D, D').
\end{eqnarray}
\end{proposition}


\begin{proof}  We begin by observing that 


\begin{eqnarray}\label{0605.11}
&   &   \|I(D) - I(D')\|_1 \\ \notag
 & = &  \sum_{S\in \mathcal P} | I_S(D) - I_S(D') | \\ \notag
 &= &  \sum_{S\in \mathcal P} \bigg|  \int_S  \left( \tilde{f}\circ \rho(D) - \tilde{f}\circ \rho(D')\right)   wdA \bigg|   \\ \notag
 &\leq  &  \sum_{S\in \mathcal P} \int_S | \tilde{f}\circ \rho(D) - \tilde{f}\circ \rho(D')|   wdA  \\ \notag 
&\leq &  \sum_{S\in \mathcal P} \,  \sum_{1\leq n \leq N} \, \int_S | f(x_n, y_n)\chi_{E_n} - f(x_n', y_n')\chi_{E_n'}| \, wdA  \\ \notag
&\leq &    \sum_{1\leq n \leq N} \, \sum_{S\in \mathcal P} \, \int_S | f(x_n, y_n)\chi_{E_n} - f(x_n', y_n')\chi_{E_n'}| \, wdA  \\ \notag
&=  &    \sum_{1\leq n \leq N} \,  \int_{\Omega_0} | f(x_n, y_n)\chi_{E_n} - f(x_n', y_n')\chi_{E_n'}| \, wdA  \
\end{eqnarray}

Let  $A$ and $B$ be two set of integers as defined in the proof of Proposition \ref{0601.A}: 
\begin{eqnarray}\label{0605.12}
A  & =  & \bigg\{n: 1\leq n \leq N,  \ \mbox{and} \ \|(x_n, y_n)-(x_n', y_n') \|_\infty  \ <  \ \frac{\la_n+\la_n'}{2}\bigg\}, \mbox{\ and}  \\ \label{0605.13}
B  & =  & \bigg\{n: 1\leq n \leq N,  \ \mbox{and} \ \|(x_n, y_n)-(x_n', y_n') \|_\infty  \ \geq \ \frac{\la_n+\la_n'}{2}\bigg\}
\end{eqnarray} 

First if $n \in B$  then 
$ \frac{\la_n+\la_n'}{2} \leq  \|(x_n, y_n)-(x_n', y_n') \|_\infty,$ and hence
\begin{eqnarray}\label{0605.15} 
 \la_n< 2\|(x_n, y_n)-(x_n', y_n') \|_\infty,  \mbox{  and  }\  \la_n' < 2\|(x_n, y_n)-(x_n', y_n') \|_\infty. 
\end{eqnarray}
Thus if $n \in B$ then by Statement (1) of Lemma \ref{0511.AA}, we have $E_n \cap E_n' = \emptyset$, and so for a  pixel $S$, we have 
\begin{eqnarray}\label{0605.16}
&   &  \int_{\Omega_0} | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}| \, wdA  \\ \notag
& \leq  &  M\|f\|_\infty \mbox{Area}(E_n ) + M \|f\|_\infty \mbox{Area}(E_n')  \\ \notag
& \leq &  M\|f\|_\infty \la_n^2+ M \|f\|_\infty {\la'}_n^2  \\ \notag
& \leq &  M\|f\|_\infty \|\la\|_\infty \la_n+ M \|f\|_\infty   \|\la\|_\infty {\la'}_n  \\ \notag
& < & 4M\|f\|_\infty \|\la\|_\infty \|(x_n, y_n)-(x_n', y_n') \|_\infty, \mbox{\ by (\ref{0605.15}).} 
\end{eqnarray}



Second, we  now focus on the integers $n \in A$, for which we use Statement (1) of Lemma \ref{0511.AA} to obtain 
\begin{eqnarray}\label{0605.17}
& & \ \ \int_{\Omega_0} | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}| \, wdA \\ \notag
&\leq & \ \ \int_{\Omega_0}\, M | f(x_n, y_n)\chi_{E_n} -   f(x_n', y_n')\chi_{E_n'}| \, dA \\ \notag
&\leq& \  \ M|f(x_n, y_n)|\mbox{Area}(E_n \setminus E_n') +  M| f(x_n', y_n')| \mbox{Area} (E_n' \setminus E_n)\ + \\ \notag
&   & + M |f(x_n, y_n) - f(x_n', y_n')| \, \mbox{Area} (E_n \cap E_n') \\ \notag
&\leq&  \ \ M\|f\|_\infty \bigg( \mbox{Area}(E_n \setminus E_n')  +  \mbox{Area}(E_n' \setminus E_n) \bigg) + \\ \notag
&   & + M |f(x_n, y_n) - f(x_n', y_n')| \, \mbox{Area} (E_n \cap E_n') \\ \notag
&\leq & \ \ M\|f\|_\infty \bigg( \mbox{Area}(E_n \setminus E_n')  +  \mbox{Area} (E_n' \setminus E_n)\bigg) + \\ \notag
&   & + M  C_f \|((x_n, y_n) - (x_n', y_n')\|_\infty \, \mbox{Area} (E_n), \mbox{ \ by (\ref{0601.100})}.  \\ \notag
&\leq & \ \ M\|f\|_\infty \bigg(  \|\la\|_\infty (C_\la +  4) \|((x_n, y_n) - (x_n', y_n')\|_\infty \bigg) + \\ \notag
&   & + M  C_f \|((x_n, y_n) - (x_n', y_n')\|_\infty \, \|\la\|_\infty^2, \mbox{ \ by (\ref{0601.15})}.  \\ \notag
&=& \ \ M \|\la\|_\infty (\|f\|_\infty (C_\la +  4) +  C_f \|\la\|_\infty) \|((x_n, y_n) - (x_n', y_n')\|_\infty  
\end{eqnarray}

Hence by putting (\ref{0605.16}) and   (\ref{0605.17}) into (\ref{0605.11}) we have 
\begin{eqnarray}\label{0605.22}
&  &  |I_S(D) - I_S(D')| \\ \notag
&\leq &  \sum_{1\leq n \leq N} \, \int_{\Omega_0} | f(x_n, y_n)\chi_{E_n} - f(x_n', y_n')\chi_{E_n'}| \, wdA  \\ \notag 
 & \leq  &  \sum_{1\leq n \leq N} C_1 \|((x_n, y_n) - (x_n', y_n')\|_\infty, \text{ where $C_1$ is given by (\ref{0605.20}).}  \\ \notag 
 &= & C_1 W_1(D, D'), 
\end{eqnarray}
\end{proof}



We have the following trivial corollary of Proposition \ref{0605.C}

%%%%%%    Corollary 4.9  %%%   


\begin{corollary}\label{0605.E}
 With the same hypotheses in Proposition \ref{0605.C}, we have 
\begin{eqnarray}\label{0605.23}
\| I(D) - I(D') \|_\infty  \leq  C_1 W_1(D, D'), 
\end{eqnarray}
\end{corollary}

\begin{proof}
Since $\|I(D) - I(D')\|_\infty \leq \|I(D) - I(D')\|_1,$ our result follows from Proposition \ref{0605.C}. 
 \end{proof}
 
  
 
In fact $\| I(D) - I(D') \|_\infty$ can be given a bound independent of $W_p(D, D')$. 

%%%%%     Corollary 4.10    %%%%%%%%%

 
 \begin{corollary}\label{0605.F}
 With the same hypotheses in Proposition \ref{0605.C}, we have 
\begin{eqnarray}\label{0605.23A}
\| I(D) - I(D') \|_\infty  \leq  2M\|f\|_\infty  \sup_{S\in \mathcal P} {\rm Area}(S).  
\end{eqnarray}
\end{corollary}

\begin{proof}  Our result follows from the following estimation.
\begin{eqnarray}\label{0606.1}
&  & \|I(D) - I(D')\|_\infty  \\ \notag
&= &  \sup_{S\in \mathcal P}  |I_S(D) - I_S(D')|   \\ \notag
& \leq & \sup_{S\in \mathcal P} \bigg| \int_S \left(\sum_{n=1}^N f(x_n, y_n) \chi_{E_n} - f(x_n', y_n') \chi_{E_n'}\right) wdA  \bigg|  \\ \notag
& \leq & \sup_{S\in \mathcal P} \,  \sum_{n=1}^N\, \int_S \, \bigg| f(x_n, y_n) \chi_{E_n} - f(x_n', y_n') \chi_{E_n'} \bigg| wdA   \\ \notag
&=& \sup_{S\in \mathcal P} \,  \sum_{n=1}^N \, \int_S \, 2\|f\|_\infty  wdA  \\ \notag
&\leq & \sup_{S\in \mathcal P} \,  \sum_{n=1}^N  \, 2M\|f\|_\infty {\rm Area}(S)  \\ \notag
&=& 2M\|f\|_\infty  \sup_{S\in \mathcal P} {\rm Area}(S).
\end{eqnarray}
\end{proof}

\end{subsection}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "arxiv_version"
%%% End:

